Inferring Data Preconditions from Deep Learning Models for Trustworthy Prediction in Deployment

Deep learning models are trained with certain assumptions about the data during the development stage and then used for prediction in the deployment stage. It is important to reason about the trustworthiness of the model's predictions with unseen data during deployment. Existing methods for specifying and verifying traditional software are insufficient for this task, as they cannot handle the complexity of DNN model architecture and expected outcomes. In this work, we propose a novel technique that uses rules derived from neural network computations to infer data preconditions for a DNN model to determine the trustworthiness of its predictions. Our approach, DeepInfer involves introducing a novel abstraction for a trained DNN model that enables weakest precondition reasoning using Dijkstra's Predicate Transformer Semantics. By deriving rules over the inductive type of neural network abstract representation, we can overcome the matrix dimensionality issues that arise from the backward non-linear computation from the output layer to the input layer. We utilize the weakest precondition computation using rules of each kind of activation function to compute layer-wise precondition from the given postcondition on the final output of a deep neural network. We extensively evaluated DeepInfer on 29 real-world DNN models using four different datasets collected from five different sources and demonstrated the utility, effectiveness, and performance improvement over closely related work. DeepInfer efficiently detects correct and incorrect predictions of high-accuracy models with high recall (0.98) and high F-1 score (0.84) and has significantly improved over prior technique, SelfChecker. The average runtime overhead of DeepInfer is low, 0.22 sec for all unseen datasets. We also compared runtime overhead using the same hardware settings and found that DeepInfer is 3.27 times faster than SelfChecker.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> challengewp.tex <==
\begin{figure*}[!h]
	\includegraphics[width=\linewidth,trim={0cm 0cm 0cm 0cm},clip]{figures/matrixwp.pdf}
	%    \includegraphics[keepaspectratio = True, scale = .4, trim={0cm 5cm 0cm 6cm},clip]{figures/BugTypes_Python.pdf}
	\footnotesize
	\caption{ Challenge involving layerwise \wpre computation } 
	%compared to original runtime of correct codes using both \deeplocalize and \umlaut Benchmark} 
	\label{fig:wpchallenge}
\end{figure*}

==> grammar.tex <==
%{grammar}, needs {obey}

%\newcommand{\heading}[1]{\vspace{3ex}{\noindent#1}\vspace{1.5ex}}
\newcommand{\goesto}{\mbox{$::=$}}
\newcommand{\arbno}[1]{#1\hbox{\rm*}}
\newcommand{\nonterm}[1]{\mbox{$\langle$#1$\rangle$}}

\newenvironment{grammar}{
  \def\:{\goesto{}}
  \def\|{$\vert$}
  \tt \myobeycr%
  \begin{tabbing}%
  \qquad \= $\vert$ \= \qquad \= \kill%
}%
{\unskip\end{tabbing}}

\newenvironment{grammar*}{
  \def\:{\goesto{}}
  \def\|{$\vert$}
  \tt%
  \begin{tabbing}%
  \qquad \= $\vert$ \= \qquad \= \kill%
}%
{\unskip\end{tabbing}}

\newenvironment{roman-grammar}{
  \def\:{\goesto{}}
  \def\|{$\vert$}
  \myobeycr%
  \begin{tabbing}%
  \qquad \= $\vert$ \= \qquad \= \hspace*{5cm} \= \qquad \= \kill%
}%
{\unskip\end{tabbing}}

\newenvironment{roman-grammar*}{
  \def\:{\goesto{}}
  \def\|{$\vert$}
  \begin{tabbing}%
  \qquad \= $\vert$ \= \qquad \= \hspace*{5cm} \= \qquad \= \kill%
}%
{\unskip\end{tabbing}}

\newenvironment{mathGrammar}{
  \def\:{\goesto{}}
  \def\|{\hbox{$\vert$}}
   \begin{displaymath}%
     \tt \obeyspaces%
}%
{\unskip\end{displaymath}}

% Commented grammars

% length before comments start on right
\newlength{\BEFOREGRAMCOMMENTLEN}
\setlength{\BEFOREGRAMCOMMENTLEN}{7cm}

% style of text inside quotations
\newcommand{\GRAMCOMMENTSTYLE}[1]{\texttt{#1}}

\newenvironment{commented-grammar}{%
\begin{grammar}%
\qquad \= $\vert$ \= \qquad \hspace*{\BEFOREGRAMCOMMENTLEN} \= \kill%
}{\end{grammar}}%

\newcommand{\gramcomment}[1]{\textrm{``\GRAMCOMMENTSTYLE{#1}''}}

% Compressed tabular grammar - takes less space
%
\newenvironment{cgrammar}{
\def\|{$\vert$}
\begin{tabular}{>{\raggedright}p{1.5cm}>{\raggedright}p{0.8cm}>{\raggedright}p{5.5cm}}%
}{\end{tabular}}%
% Production takes three parameters
% name, start symbol, production
% TODO: Extend using ithen package so that it is only defined within the cgrammar
% package.
\newcommand{\production}[3]{\mbox{#1} & \nonterm{#2}~\goesto & #3 \tabularnewline}


==> obey.tex <==
%{obey}

% \myobeycr is same as \obeycr, but doesn't do a \@gobblecr.
{\catcode`\^^M=13 \gdef\myobeycr{\catcode`\^^M=13 \def^^M{\\}}%
\gdef\restorecr{\catcode`\^^M=5 }}

% \obeytabs
{\catcode`\^^I=13 \gdef\obeytabs{\catcode`\^^I=13 \def^^I{\hbox{\hskip 4em}}}}

% \obeyspaces
{\obeyspaces\gdef {\hbox{\hskip0.5em}}}

% environment for displayed text, indented, obeys cr, tab, spaces
\newenvironment{obeyDisplay}{%
\samepage%
\begin{list}{}{}\item\obeyspaces\obeytabs\obeycr}{%
\end{list}}


==> tables/oldTables.tex <==
%RQ1 tables
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table*}[]
% \tiny
%   \centering
%   \caption{Experiment with PIMA dataset}
% \begin{tabular}{|ll|
% >{\columncolor[HTML]{00FF00}}r 
% >{\columncolor[HTML]{00FF00}}c |rc|
% >{\columncolor[HTML]{00FF00}}r 
% >{\columncolor[HTML]{00FF00}}c |rc|
% >{\columncolor[HTML]{00FF00}}r 
% >{\columncolor[HTML]{00FF00}}c |rc|
% >{\columncolor[HTML]{00FF00}}r 
% >{\columncolor[HTML]{00FF00}}c |rc|}
% \hline
% \multicolumn{1}{|l|}{}                                                   & \textbf{}             & \multicolumn{2}{c|}{\cellcolor[HTML]{F3F3F3}\#1}                                                           & \multicolumn{2}{c|}{\cellcolor[HTML]{FFFFFF}\#2}                                                           & \multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}\#3}                                                           & \multicolumn{2}{c|}{\cellcolor[HTML]{FFFFFF}\#4}                                                           & \multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}\#5}                                                           & \multicolumn{2}{c|}{\#6}                                                                                   & \multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}\#7}                                                         & \multicolumn{2}{c|}{\#8}                                                                                           \\ \cline{2-18} 
% \multicolumn{1}{|l|}{\multirow{-2}{*}{\textbf{Features}}}                & \textbf{Precondition} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}Value}   & \cellcolor[HTML]{F3F3F3}Sat?                        & \multicolumn{1}{l|}{Value}                           & Sat?                                                & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}Value}   & \cellcolor[HTML]{EFEFEF}Sat?                        & \multicolumn{1}{l|}{Value}                           & Sat?                                                & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}Value}   & \cellcolor[HTML]{EFEFEF}Sat?                        & \multicolumn{1}{l|}{Value}                           & Sat?                                                & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}Value} & \cellcolor[HTML]{EFEFEF}Sat?                        & \multicolumn{1}{l|}{Value}                          & Sat?                                                         \\ \hline
% \multicolumn{1}{|l|}{\cellcolor[HTML]{00FF00}\#Pregnancies}              & X \textgreater -0.56  & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}6.00}    & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}1.00}    & \cellcolor[HTML]{00FF00}Y                           & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}8.00}    & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}1.00}    & \cellcolor[HTML]{00FF00}Y                           & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}0.00}    & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}5.00}    & \cellcolor[HTML]{00FF00}Y                           & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}3.00}  & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}10.00}  & \cellcolor[HTML]{00FF00}Y                                    \\ \hline
% \multicolumn{1}{|l|}{\cellcolor[HTML]{00FF00}Glucose}                    & X \textgreater 0.86   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}148.00}  & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}85.00}   & \cellcolor[HTML]{00FF00}Y                           & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}183.00}  & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}89.00}   & \cellcolor[HTML]{00FF00}Y                           & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}137.00}  & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}116.00}  & \cellcolor[HTML]{00FF00}Y                           & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}78.00} & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}115.00} & \cellcolor[HTML]{00FF00}Y                                    \\ \hline
% \multicolumn{1}{|l|}{\cellcolor[HTML]{FF0000}Blood Pressure}             & X \textgreater 1.29   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}72.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}66.00}   & \cellcolor[HTML]{00FF00}Y                           & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}64.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}66.00}   & \cellcolor[HTML]{00FF00}Y                           & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}40.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}74.00}   & \cellcolor[HTML]{00FF00}Y                           & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}50.00} & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}0.00}   & \cellcolor[HTML]{FF0000}N                                    \\ \hline
% \multicolumn{1}{|l|}{\cellcolor[HTML]{00FF00}Skin Thickness}             & X \textgreater -8.21  & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}35.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}29.00}   & \cellcolor[HTML]{00FF00}Y                           & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}0.00}    & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}23.00}   & \cellcolor[HTML]{00FF00}Y                           & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}35.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}0.00}    & \cellcolor[HTML]{00FF00}Y                           & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}32.00} & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}0.00}   & \cellcolor[HTML]{00FF00}Y                                    \\ \hline
% \multicolumn{1}{|l|}{\cellcolor[HTML]{FF0000}Insulin}                    & X \textgreater 0.24   & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}0.00}    & \cellcolor[HTML]{FF0000}N                           & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}0.00}    & \cellcolor[HTML]{FF0000}N                           & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}0.00}    & \cellcolor[HTML]{FF0000}N                           & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}94.00}   & \cellcolor[HTML]{00FF00}Y                           & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}168.00}  & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}0.00}    & \cellcolor[HTML]{FF0000}N                           & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}88.00} & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}0.00}   & \cellcolor[HTML]{FF0000}N                                    \\ \hline
% \multicolumn{1}{|l|}{\cellcolor[HTML]{00FF00}BMI}                        & X \textgreater -1.37  & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}33.60}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}26.60}   & \cellcolor[HTML]{00FF00}Y                           & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}23.30}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}28.10}   & \cellcolor[HTML]{00FF00}Y                           & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}43.10}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}25.60}   & \cellcolor[HTML]{00FF00}Y                           & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}31.00} & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}35.30}  & \cellcolor[HTML]{00FF00}Y                                    \\ \hline
% \multicolumn{1}{|l|}{\cellcolor[HTML]{FF0000}Diabetes Pedigree function} & X \textgreater 0.49   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}0.63}    & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}0.35}    & \cellcolor[HTML]{FF0000}N                           & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}0.63}    & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}0.17}    & \cellcolor[HTML]{FF0000}N                           & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}2.28}    & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}0.20}    & \cellcolor[HTML]{FF0000}N                           & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}0.25}  & \cellcolor[HTML]{FF0000}N                           & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}0.13}   & \cellcolor[HTML]{FF0000}N                                    \\ \hline
% \multicolumn{1}{|l|}{\cellcolor[HTML]{00FF00}Age}                        & X \textgreater 0.80   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}50.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}31.00}   & \cellcolor[HTML]{00FF00}Y                           & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}32.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}21.00}   & \cellcolor[HTML]{00FF00}Y                           & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}33.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}30.00}   & \cellcolor[HTML]{00FF00}Y                           & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}26.00} & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}29.00}  & \cellcolor[HTML]{00FF00}Y                                    \\ \hline
% \multicolumn{2}{|l|}{Prediction}                                                                 & \multicolumn{1}{l|}{\cellcolor[HTML]{D9EAD3}Correct} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9EAD3}1 ( 1)} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9EAD3}Correct} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9EAD3}0 ( 0)} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9EAD3}Correct} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9EAD3}1 ( 1)} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9EAD3}Correct} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9EAD3}0 ( 0)} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9EAD3}Correct} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9EAD3}1 ( 1)} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9EAD3}Correct} & \multicolumn{1}{l|}{\cellcolor[HTML]{D9EAD3}0 ( 0)} & \multicolumn{1}{l|}{\cellcolor[HTML]{F4CCCC}Wrong} & \multicolumn{1}{l|}{\cellcolor[HTML]{F4CCCC}0 ( 1)} & \multicolumn{1}{l|}{\cellcolor[HTML]{F4CCCC}Wrong}  & \multicolumn{1}{l|}{\cellcolor[HTML]{F4CCCC}\textbf{1 ( 0)}} \\ \hline
% \end{tabular}
% \end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table*}[]
% \tiny
%   \centering
%   \caption{Missing value Experiment with PIMA dataset}
% \begin{tabular}{|lc|rc|rc|rc|rc|rc|rc|rc|rc|}
% \hline
% \multicolumn{1}{|l|}{}                                                   & \multicolumn{1}{l|}{\textbf{}}                  & \multicolumn{2}{c|}{\cellcolor[HTML]{F3F3F3}\#1}                                                           & \multicolumn{2}{c|}{\cellcolor[HTML]{FFFFFF}\#2}                                                           & \multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}\#3}                                                           & \multicolumn{2}{c|}{\cellcolor[HTML]{FFFFFF}\#4}                                                           & \multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}\#5}                                                           & \multicolumn{2}{c|}{\#6}                                                                                   & \multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}\#7}                                                                  & \multicolumn{2}{c|}{\#8}                                                                                   \\ \cline{2-18} 
% \multicolumn{1}{|l|}{\multirow{-2}{*}{\textbf{Features}}}                & \textbf{Precondition}                           & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}Value}   & \cellcolor[HTML]{F3F3F3}Sat?                        & \multicolumn{1}{r|}{Value}                           & Sat?                                                & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}Value}   & \cellcolor[HTML]{EFEFEF}Sat?                        & \multicolumn{1}{r|}{Value}                           & Sat?                                                & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}Value}   & \cellcolor[HTML]{EFEFEF}Sat?                        & \multicolumn{1}{r|}{Value}                           & Sat?                                                & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}Value} & \cellcolor[HTML]{EFEFEF}Sat?                                 & \multicolumn{1}{r|}{Value}                           & Sat?                                                \\ \hline
% \rowcolor[HTML]{00FF00} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{00FF00}\#Pregnancies}              & \cellcolor[HTML]{CFE2F3}X \textgreater{}= -4.93 & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}6.00}    & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}1.00}    & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}8.00}    & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}1.00}    & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}0.00}    & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}5.00}    & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}3.00}  & Y                                                            & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}10.00}   & Y                                                   \\ \hline
% \rowcolor[HTML]{00FF00} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{00FF00}Glucose}                    & \cellcolor[HTML]{CFE2F3}X \textgreater{}=-1.15  & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}148.00}  & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}85.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}183.00}  & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}89.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}137.00}  & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}116.00}  & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}78.00} & Y                                                            & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}115.00}  & Y                                                   \\ \hline
% \rowcolor[HTML]{00FF00} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{00FF00}Blood Pressure}             & \cellcolor[HTML]{CFE2F3}X \textgreater{}=-0.14  & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}72.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}66.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}64.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}66.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}40.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}74.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}50.00} & Y                                                            & \multicolumn{1}{r|}{\cellcolor[HTML]{00FFFF}72.65}   & Y                                                   \\ \hline
% \rowcolor[HTML]{00FF00} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{00FF00}Skin Thickness}             & \cellcolor[HTML]{CFE2F3}X \textgreater{}=-36.93 & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}35.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}29.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FFFF}29.31}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}23.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}35.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FFFF}29.31}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}32.00} & Y                                                            & \multicolumn{1}{r|}{\cellcolor[HTML]{00FFFF}29.31}   & Y                                                   \\ \hline
% \rowcolor[HTML]{00FF00} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{00FF00}Insulin}                    & \cellcolor[HTML]{CFE2F3}X \textgreater{}=-2.71  & \multicolumn{1}{r|}{\cellcolor[HTML]{00FFFF}157.60}  & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FFFF}157.60}  & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FFFF}157.60}  & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}94.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}168.00}  & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FFFF}157.60}  & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}88.00} & Y                                                            & \multicolumn{1}{r|}{\cellcolor[HTML]{00FFFF}157.60}  & Y                                                   \\ \hline
% \rowcolor[HTML]{00FF00} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{00FF00}BMI}                        & \cellcolor[HTML]{CFE2F3}X \textgreater{}=-7.37  & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}33.60}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}26.60}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}23.30}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}28.10}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}43.10}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}25.60}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}31.00} & Y                                                            & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}35.30}   & Y                                                   \\ \hline
% \rowcolor[HTML]{00FF00} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{00FF00}Diabetes Pedigree function} & \cellcolor[HTML]{CFE2F3}X \textgreater{}=-2.07  & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}0.63}    & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}0.35}    & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}0.63}    & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}0.17}    & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}2.28}    & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}0.20}    & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}0.25}  & Y                                                            & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}0.13}    & Y                                                   \\ \hline
% \rowcolor[HTML]{00FF00} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{00FF00}Age}                        & \cellcolor[HTML]{CFE2F3}X \textgreater{}=-1.31  & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}50.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}31.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}32.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}21.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}33.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}30.00}   & Y                                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}26.00} & Y                                                            & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}29.00}   & Y                                                   \\ \hline
% \multicolumn{2}{|l|}{\textbf{Prediction}}                                                                                  & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}Correct} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}1 ( 1)} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}Correct} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}0 ( 0)} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}Correct} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}1 ( 1)} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}Correct} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}0 ( 0)} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}Correct} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}1 ( 1)} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}Correct} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}0 ( 0)} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}Wrong} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}\textbf{0 ( 1)}} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}Correct} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}0 ( 0)} \\ \hline
% \end{tabular}
% \end{table*}

% % Table generated by Excel2LaTeX from sheet 'Example1layer_PIMA'
% %\begin{sidewaystable*}[htbp]
% % \begin{table*}[htbp]
% % \tiny
% %   \centering
% %   \caption{eeriment with PIMA dataset}
% %     \begin{tabular}{rrllllllllllllllll}
% %     \hline
% %     \multicolumn{1}{|r|}{\multirow{2}[4]{*}{\textbf{Features}}} & \multicolumn{1}{l|}{\textbf{ }} & \multicolumn{2}{l|}{\cellcolor[rgb]{ .953,  .953,  .953}Ex \#1} & \multicolumn{1}{l|}{Ex \#2} & \multicolumn{1}{l|}{} & \multicolumn{2}{l|}{\cellcolor[rgb]{ .937,  .937,  .937}Ex \#3} & \multicolumn{1}{l|}{Ex \#4} & \multicolumn{1}{r|}{} & \multicolumn{2}{l|}{\cellcolor[rgb]{ .937,  .937,  .937}Ex \#5} & \multicolumn{2}{l|}{Ex \#6} & \multicolumn{2}{l|}{\cellcolor[rgb]{ .937,  .937,  .937}Ex \#7} & \multicolumn{2}{l|}{Ex \#8} \\
% % \cline{2-18}    \multicolumn{1}{|r|}{} & \multicolumn{1}{l|}{\textbf{Precondition }} & \multicolumn{1}{l|}{\cellcolor[rgb]{ .953,  .953,  .953}Value} & \multicolumn{1}{l|}{\cellcolor[rgb]{ .953,  .953,  .953}Sat?} & \multicolumn{1}{l|}{Value} & \multicolumn{1}{l|}{Sat?} & \multicolumn{1}{l|}{\cellcolor[rgb]{ .937,  .937,  .937}Value} & \multicolumn{1}{l|}{\cellcolor[rgb]{ .937,  .937,  .937}Sat?} & \multicolumn{1}{l|}{Value} & \multicolumn{1}{l|}{Sat?} & \multicolumn{1}{l|}{\cellcolor[rgb]{ .937,  .937,  .937}Value} & \multicolumn{1}{l|}{\cellcolor[rgb]{ .937,  .937,  .937}Sat?} & \multicolumn{1}{l|}{Value} & \multicolumn{1}{l|}{Sat?} & \multicolumn{1}{l|}{\cellcolor[rgb]{ .937,  .937,  .937}Value} & \multicolumn{1}{l|}{\cellcolor[rgb]{ .937,  .937,  .937}Sat?} & \multicolumn{1}{l|}{Value} & \multicolumn{1}{l|}{Sat?} \\
% %     \hline
% %     \rowcolor[rgb]{ 0,  1,  0} \multicolumn{1}{|l|}{\#Pregnancies} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}X $\ge$ -0.56} & \multicolumn{1}{r|}{6.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{1.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{8.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{1.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{0.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{5.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{3.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{10.00} & \multicolumn{1}{l|}{Y} \\
% %     \hline
% %     \rowcolor[rgb]{ 0,  1,  0} \multicolumn{1}{|l|}{Glucose} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}X $\ge$ 0.86} & \multicolumn{1}{r|}{148.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{85.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{183.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{89.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{137.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{116.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{78.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{115.00} & \multicolumn{1}{l|}{Y} \\
% %     \hline
% %     \rowcolor[rgb]{ 1,  0,  0} \multicolumn{1}{|l|}{Blood Pressure} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}X $\ge$ 1.29} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 0,  1,  0}72.00} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 0,  1,  0}Y} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 0,  1,  0}66.00} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 0,  1,  0}Y} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 0,  1,  0}64.00} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 0,  1,  0}Y} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 0,  1,  0}66.00} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 0,  1,  0}Y} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 0,  1,  0}40.00} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 0,  1,  0}Y} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 0,  1,  0}74.00} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 0,  1,  0}Y} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 0,  1,  0}50.00} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 0,  1,  0}Y} & \multicolumn{1}{r|}{0.00} & \multicolumn{1}{l|}{N} \\
% %     \hline
% %     \rowcolor[rgb]{ 0,  1,  0} \multicolumn{1}{|l|}{Skin Thickness} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}X $\ge$ -8.21} & \multicolumn{1}{r|}{35.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{29.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{0.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{23.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{35.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{0.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{32.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{0.00} & \multicolumn{1}{l|}{Y} \\
% %     \hline
% %     \rowcolor[rgb]{ 1,  0,  0} \multicolumn{1}{|l|}{Insulin} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}X $\ge$ 0.24} & \multicolumn{1}{r|}{0.00} & \multicolumn{1}{l|}{N} & \multicolumn{1}{r|}{0.00} & \multicolumn{1}{l|}{N} & \multicolumn{1}{r|}{0.00} & \multicolumn{1}{l|}{N} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 0,  1,  0}94.00} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 0,  1,  0}Y} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 0,  1,  0}168.00} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 0,  1,  0}Y} & \multicolumn{1}{r|}{0.00} & \multicolumn{1}{l|}{N} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 0,  1,  0}88.00} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 0,  1,  0}Y} & \multicolumn{1}{r|}{0.00} & \multicolumn{1}{l|}{N} \\
% %     \hline
% %     \rowcolor[rgb]{ 0,  1,  0} \multicolumn{1}{|l|}{BMI} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}X $\ge$ -1.37} & \multicolumn{1}{r|}{33.60} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{26.60} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{23.30} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{28.10} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{43.10} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{25.60} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{31.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{35.30} & \multicolumn{1}{l|}{Y} \\
% %     \hline
% %     \rowcolor[rgb]{ 1,  0,  0} \multicolumn{1}{|l|}{Diabetes Pedigree function} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}X $\ge$ 0.49} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 0,  1,  0}0.63} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 0,  1,  0}Y} & \multicolumn{1}{r|}{0.35} & \multicolumn{1}{l|}{N} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 0,  1,  0}0.63} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 0,  1,  0}Y} & \multicolumn{1}{r|}{0.17} & \multicolumn{1}{l|}{N} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 0,  1,  0}2.28} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 0,  1,  0}Y} & \multicolumn{1}{r|}{0.20} & \multicolumn{1}{l|}{N} & \multicolumn{1}{r|}{0.25} & \multicolumn{1}{l|}{N} & \multicolumn{1}{r|}{0.13} & \multicolumn{1}{l|}{N} \\
% %     \hline
% %     \rowcolor[rgb]{ 0,  1,  0} \multicolumn{1}{|l|}{Age} & \multicolumn{1}{l|}{\cellcolor[rgb]{ 1,  1,  1}X $\ge$ 0.80} & \multicolumn{1}{r|}{50.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{31.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{32.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{21.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{33.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{30.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{26.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{29.00} & \multicolumn{1}{l|}{Y} \\
% %     \hline
% %           &       & \cellcolor[rgb]{ .851,  .918,  .827}Correct Prediction & \cellcolor[rgb]{ .851,  .918,  .827}1 (1) & \cellcolor[rgb]{ .851,  .918,  .827}Correct Prediction & \cellcolor[rgb]{ .851,  .918,  .827}0 (0) & \cellcolor[rgb]{ .851,  .918,  .827}Correct Prediction & \cellcolor[rgb]{ .851,  .918,  .827}1 (e 1) & \cellcolor[rgb]{ .851,  .918,  .827}Correct Prediction & \cellcolor[rgb]{ .851,  .918,  .827}0 (0) & \cellcolor[rgb]{ .851,  .918,  .827}Correct Prediction & \cellcolor[rgb]{ .851,  .918,  .827}1 (1) & \cellcolor[rgb]{ .851,  .918,  .827}Correct Prediction & \cellcolor[rgb]{ .851,  .918,  .827}0 (e 0) & \cellcolor[rgb]{ .957,  .8,  .8}Wrong Prediction & \cellcolor[rgb]{ .957,  .8,  .8}\textbf{0 (1)} & \cellcolor[rgb]{ .957,  .8,  .8}Wrong Prediction & \cellcolor[rgb]{ .957,  .8,  .8}\textbf{1 (0)} \\
% %     \end{tabular}%
% %   \label{tab:pima1}%
% % %\end{sidewaystable*}
% % \end{table*}%


% % Table generated by Excel2LaTeX from sheet 'Example1layer_PIMA'
% % \begin{table*}
% % %\begin{table}[htbp]
% % \tiny
% %   \centering
% %   \caption{Missing Value eeriment with PIMA dataset}
% %     \begin{tabular}{rrllllllllllllllll}
% %     \hline
% %     \multicolumn{1}{|r|}{\multirow{2}[4]{*}{\textbf{Features}}} & \multicolumn{1}{l|}{\textbf{ }} & \multicolumn{2}{l|}{\cellcolor[rgb]{ .953,  .953,  .953}Ex \#1} & \multicolumn{1}{l|}{Ex \#2} & \multicolumn{1}{l|}{} & \multicolumn{2}{l|}{\cellcolor[rgb]{ .937,  .937,  .937}Ex \#3} & \multicolumn{1}{l|}{Ex \#4} & \multicolumn{1}{r|}{} & \multicolumn{2}{l|}{\cellcolor[rgb]{ .937,  .937,  .937}Ex \#5} & \multicolumn{2}{l|}{Ex \#6} & \multicolumn{2}{l|}{\cellcolor[rgb]{ .937,  .937,  .937}Ex \#7} & \multicolumn{2}{l|}{Ex \#8} \\
% % \cline{2-18}    \multicolumn{1}{|r|}{} & \multicolumn{1}{l|}{\textbf{Precondition }} & \multicolumn{1}{l|}{\cellcolor[rgb]{ .953,  .953,  .953}Value} & \multicolumn{1}{l|}{\cellcolor[rgb]{ .953,  .953,  .953}Sat?} & \multicolumn{1}{l|}{Value} & \multicolumn{1}{l|}{Sat?} & \multicolumn{1}{l|}{\cellcolor[rgb]{ .937,  .937,  .937}Value} & \multicolumn{1}{l|}{\cellcolor[rgb]{ .937,  .937,  .937}Sat?} & \multicolumn{1}{l|}{Value} & \multicolumn{1}{l|}{Sat?} & \multicolumn{1}{l|}{\cellcolor[rgb]{ .937,  .937,  .937}Value} & \multicolumn{1}{l|}{\cellcolor[rgb]{ .937,  .937,  .937}Sat?} & \multicolumn{1}{l|}{Value} & \multicolumn{1}{l|}{Sat?} & \multicolumn{1}{l|}{\cellcolor[rgb]{ .937,  .937,  .937}Value} & \multicolumn{1}{l|}{\cellcolor[rgb]{ .937,  .937,  .937}Sat?} & \multicolumn{1}{l|}{Value} & \multicolumn{1}{l|}{Sat?} \\
% %     \hline
% %     \rowcolor[rgb]{ 0,  1,  0} \multicolumn{1}{|l|}{\#Pregnancies} & \multicolumn{1}{l|}{\cellcolor[rgb]{ .812,  .886,  .953}X >= -4.93} & \multicolumn{1}{r|}{6.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{1.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{8.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{1.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{0.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{5.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{3.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{10.00} & \multicolumn{1}{l|}{Y} \\
% %     \hline
% %     \rowcolor[rgb]{ 0,  1,  0} \multicolumn{1}{|l|}{Glucose} & \multicolumn{1}{l|}{\cellcolor[rgb]{ .812,  .886,  .953}X >=-1.15} & \multicolumn{1}{r|}{148.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{85.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{183.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{89.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{137.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{116.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{78.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{115.00} & \multicolumn{1}{l|}{Y} \\
% %     \hline
% %     \rowcolor[rgb]{ 0,  1,  0} \multicolumn{1}{|l|}{Blood Pressure} & \multicolumn{1}{l|}{\cellcolor[rgb]{ .812,  .886,  .953}X >=-0.14} & \multicolumn{1}{r|}{72.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{66.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{64.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{66.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{40.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{74.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{50.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 0,  1,  1}72.65} & \multicolumn{1}{l|}{Y} \\
% %     \hline
% %     \rowcolor[rgb]{ 0,  1,  0} \multicolumn{1}{|l|}{Skin Thickness} & \multicolumn{1}{l|}{\cellcolor[rgb]{ .812,  .886,  .953}X >=-36.93} & \multicolumn{1}{r|}{35.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{29.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 0,  1,  1}29.31} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{23.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{35.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 0,  1,  1}29.31} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{32.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 0,  1,  1}29.31} & \multicolumn{1}{l|}{Y} \\
% %     \hline
% %     \rowcolor[rgb]{ 0,  1,  0} \multicolumn{1}{|l|}{Insulin} & \multicolumn{1}{l|}{\cellcolor[rgb]{ .812,  .886,  .953}X >=-2.71} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 0,  1,  1}157.60} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 0,  1,  1}157.60} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 0,  1,  1}157.60} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{94.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{168.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 0,  1,  1}157.60} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{88.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 0,  1,  1}157.60} & \multicolumn{1}{l|}{Y} \\
% %     \hline
% %     \rowcolor[rgb]{ 0,  1,  0} \multicolumn{1}{|l|}{BMI} & \multicolumn{1}{l|}{\cellcolor[rgb]{ .812,  .886,  .953}X >=-7.37} & \multicolumn{1}{r|}{33.60} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{26.60} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{23.30} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{28.10} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{43.10} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{25.60} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{31.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{35.30} & \multicolumn{1}{l|}{Y} \\
% %     \hline
% %     \rowcolor[rgb]{ 0,  1,  0} \multicolumn{1}{|l|}{Diabetes Pedigree function} & \multicolumn{1}{l|}{\cellcolor[rgb]{ .812,  .886,  .953}X >=-2.07} & \multicolumn{1}{r|}{0.63} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{0.35} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{0.63} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{0.17} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{2.28} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{0.20} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{0.25} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{0.13} & \multicolumn{1}{l|}{Y} \\
% %     \hline
% %     \rowcolor[rgb]{ 0,  1,  0} \multicolumn{1}{|l|}{Age} & \multicolumn{1}{l|}{\cellcolor[rgb]{ .812,  .886,  .953}X >=-1.31} & \multicolumn{1}{r|}{50.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{31.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{32.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{21.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{33.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{30.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{26.00} & \multicolumn{1}{l|}{Y} & \multicolumn{1}{r|}{29.00} & \multicolumn{1}{l|}{Y} \\
% %     \hline
% %           &       & \cellcolor[rgb]{ .851,  .918,  .827}Correct Prediction & \cellcolor[rgb]{ .851,  .918,  .827}1 (e 1) & \cellcolor[rgb]{ .851,  .918,  .827}Correct Prediction & \cellcolor[rgb]{ .851,  .918,  .827}0 (e 0) & \cellcolor[rgb]{ .851,  .918,  .827}Correct Prediction & \cellcolor[rgb]{ .851,  .918,  .827}1 (e 1) & \cellcolor[rgb]{ .851,  .918,  .827}Correct Prediction & \cellcolor[rgb]{ .851,  .918,  .827}0 (e 0) & \cellcolor[rgb]{ .851,  .918,  .827}Correct Prediction & \cellcolor[rgb]{ .851,  .918,  .827}1 (e 1) & \cellcolor[rgb]{ .851,  .918,  .827}Correct Prediction & \cellcolor[rgb]{ .851,  .918,  .827}0 (e 0) & \cellcolor[rgb]{ .957,  .8,  .8}Wrong Prediction & \cellcolor[rgb]{ .957,  .8,  .8}\textbf{0 (e 1)} & \cellcolor[rgb]{ .851,  .918,  .827}Correct Prediction & \cellcolor[rgb]{ .851,  .918,  .827}0 (e 0) \\
% %     \end{tabular}%
% %   \label{tab:pima2}%
% %   \end{table*}
% % %\end{table}%



% % Titanic dataset example

% % Please add the following required packages to your document preamble:
% % \usepackage[table,xcdraw]{xcolor}
% % If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table*}[]
% \tiny
%   \centering
%   \caption{Experiment with Titanic dataset}
% \begin{tabular}{|ll|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|}
% \hline
% \multicolumn{1}{|l|}{}                                  & \textbf{}                                       & \multicolumn{2}{c|}{\cellcolor[HTML]{F3F3F3}\#1}                                       & \multicolumn{2}{c|}{\cellcolor[HTML]{FFFFFF}\#2}                                    & \multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}\#3}                                       & \multicolumn{2}{c|}{\cellcolor[HTML]{FFFFFF}\#4}                                    & \multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}\#5}                                       & \multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}\#6}                                       & \multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}\#7}                                       & \multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}\#8}                                       & \multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}\#9}                                       & \multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}\#10}                                                          \\ \hline
% \multicolumn{1}{|l|}{\textbf{Features}}                 & \textbf{Precondition}                           & \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}Value}      & \cellcolor[HTML]{F3F3F3}Sat? & \multicolumn{1}{c|}{Value}                              & Sat?                      & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Value}      & \cellcolor[HTML]{EFEFEF}Sat? & \multicolumn{1}{c|}{Value}                              & Sat?                      & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Value}      & \cellcolor[HTML]{EFEFEF}Sat? & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Value}      & \cellcolor[HTML]{EFEFEF}Sat? & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Value}      & \cellcolor[HTML]{EFEFEF}Sat? & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Value}      & \cellcolor[HTML]{EFEFEF}Sat? & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Value}      & \cellcolor[HTML]{EFEFEF}Sat? & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Value}      & \cellcolor[HTML]{EFEFEF}Sat?                     \\ \hline
% \rowcolor[HTML]{00FF00} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{00FF00}Pclass}    & \cellcolor[HTML]{F3F3F3}X \textgreater{}= -0.10 & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}\textbf{3}} & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}\textbf{3}} & Y                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}\textbf{2}} & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}\textbf{3}} & Y                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}\textbf{3}} & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}\textbf{3}} & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}\textbf{3}} & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}\textbf{2}} & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}\textbf{3}} & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}\textbf{3}} & Y                                                \\ \hline
% \rowcolor[HTML]{FF0000} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{FF0000}Gender}    & \cellcolor[HTML]{F3F3F3}X \textgreater{}= 0.05  & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & \cellcolor[HTML]{00FF00}Y & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & \cellcolor[HTML]{00FF00}Y    & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & \cellcolor[HTML]{00FF00}Y    & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & \cellcolor[HTML]{00FF00}Y    & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                                                \\ \hline
% \rowcolor[HTML]{FF0000} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{FF0000}Master}    & \cellcolor[HTML]{F3F3F3}X \textgreater{}= 0.05  & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                                                \\ \hline
% \rowcolor[HTML]{00FF00} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{00FF00}Miss}      & \cellcolor[HTML]{F3F3F3}X \textgreater{}= -0.02 & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                                                \\ \hline
% \rowcolor[HTML]{00FF00} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{00FF00}Mr}        & \cellcolor[HTML]{F3F3F3}X \textgreater{}= -0.11 & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & Y                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & Y                                                \\ \hline
% \rowcolor[HTML]{00FF00} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{00FF00}Mrs}       & \cellcolor[HTML]{F3F3F3}X \textgreater{}= -0.12 & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & Y                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                                                \\ \hline
% \rowcolor[HTML]{00FF00} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{00FF00}Others}    & \cellcolor[HTML]{F3F3F3}X \textgreater{}= -0.06 & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                                                \\ \hline
% \rowcolor[HTML]{00FF00} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{00FF00}Family}    & \cellcolor[HTML]{F3F3F3}X \textgreater{}= 0.06  & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}2}          & Y                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & Y                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}3}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}3}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}3}          & Y                                                \\ \hline
% \rowcolor[HTML]{00FF00} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{00FF00}Fare-bin}  & \cellcolor[HTML]{F3F3F3}X \textgreater{}= 0.01  & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & Y                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}2}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}2}          & Y                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}3}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}2}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}4}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}4}          & Y                                                \\ \hline
% \rowcolor[HTML]{00FF00} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{00FF00}Age-bin}   & \cellcolor[HTML]{F3F3F3}X \textgreater{}= -0.12 & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}5}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}5}          & Y                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}6}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}4}          & Y                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}4}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}3}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}4}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}4}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}3}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}4}          & Y                                                \\ \hline
% \rowcolor[HTML]{FF0000} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{FF0000}Ticket\_1} & \cellcolor[HTML]{F3F3F3}X \textgreater{}= 0.01  & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}N}   \\ \hline
% \rowcolor[HTML]{00FF00} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{00FF00}Ticket\_2} & \cellcolor[HTML]{F3F3F3}X \textgreater{}= -0.10 & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}Y}   \\ \hline
% \rowcolor[HTML]{FF0000} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{FF0000}Ticket\_3} & \cellcolor[HTML]{F3F3F3}X \textgreater{}= 0.03  & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & \cellcolor[HTML]{00FF00}Y    & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & \cellcolor[HTML]{00FF00}Y & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & \cellcolor[HTML]{00FF00}Y & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & \cellcolor[HTML]{00FF00}Y    & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & \cellcolor[HTML]{00FF00}Y    & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}N}   \\ \hline
% \rowcolor[HTML]{FF0000} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{FF0000}Ticket\_4} & \cellcolor[HTML]{F3F3F3}X \textgreater{}= 0.01  & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & \cellcolor[HTML]{00FF00}Y    & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}1}          & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}Y}   \\ \hline
% \rowcolor[HTML]{FF0000} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{FF0000}Ticket\_C} & \cellcolor[HTML]{F3F3F3}X \textgreater{}= 0.10  & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & N                            & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}N}   \\ \hline
% \rowcolor[HTML]{00FF00} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{00FF00}Ticket\_P} & \cellcolor[HTML]{F3F3F3}X \textgreater{}= -0.11 & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}Y}   \\ \hline
% \rowcolor[HTML]{00FF00} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{00FF00}Ticket\_S} & \cellcolor[HTML]{F3F3F3}X \textgreater{}= -0.01 & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & Y                            & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}Y}   \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% \multicolumn{2}{|l|}{\cellcolor[HTML]{EFEFEF}Prediction}                                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{0}} & N S                          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{1}} & S                         & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{0}} & N S                          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{0}} & N S                       & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{1}} & S                            & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{0}} & N S                          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{1}} & S                            & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{0}} & N S                          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{1}} & S                            & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}N S} \\ \hline
% \end{tabular}
% \end{table*}






% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table*}[htbp]
% \tiny
%   \centering
%   \caption{Experiment with house price prediction dataset}
% \begin{tabular}{|l|l|rl|rl|rl|rl|rl|}
% \hline
%                                                                                          & \textbf{}                                     & \multicolumn{2}{c|}{\cellcolor[HTML]{F3F3F3}\#1}                                   & \multicolumn{2}{c|}{\cellcolor[HTML]{FFFFFF}\#2}                                  & \multicolumn{2}{c|}{\#3}                                                          & \multicolumn{2}{c|}{\#4}                                                           & \multicolumn{2}{c|}{\#5}                                                           \\ \cline{2-12} 
% \multirow{-2}{*}{\textbf{Features}}                                                      & \textbf{Precondition}                         & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}Value}  & \cellcolor[HTML]{F3F3F3}Sat? & \multicolumn{1}{l|}{Value}                          & Sat?                        & \multicolumn{1}{l|}{Value}                          & Sat?                        & \multicolumn{1}{l|}{Value}                           & Sat?                        & \multicolumn{1}{l|}{Value}                           & Sat?                        \\ \hline
% CRIM    per capita crime rate by town                                                    & \cellcolor[HTML]{FF0000}\textgreater{}= 1.75  & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}0.64}   & \cellcolor[HTML]{FF0000}No   & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}1.05}   & \cellcolor[HTML]{FF0000}No  & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}0.01}   & \cellcolor[HTML]{FF0000}No  & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}0.15445} & \cellcolor[HTML]{FF0000}No  & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}0.10328} & \cellcolor[HTML]{FF0000}No  \\ \hline
% ZN        proportion of residential land zoned for lots over 25,000 sq.ft.               & \cellcolor[HTML]{00FF00}\textgreater{}= -0.88 & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}0.00}   & \cellcolor[HTML]{00FF00}Yes  & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}0.00}   & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}100.00} & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}25}      & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}25}      & \cellcolor[HTML]{00FF00}Yes \\ \hline
% INDUS   proportion of non-retail business acres per town                                 & \cellcolor[HTML]{00FF00}\textgreater{}= 5.00  & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}8.14}   & \cellcolor[HTML]{00FF00}Yes  & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}8.14}   & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}1.32}   & \cellcolor[HTML]{FF0000}No  & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}5.13}    & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}5.13}    & \cellcolor[HTML]{00FF00}Yes \\ \hline
% CHAS     Charles River dummy variable (= 1 if tract bounds river; 0 otherwise)           & \cellcolor[HTML]{FF0000}\textgreater{}= 2.97  & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}0.00}   & \cellcolor[HTML]{FF0000}No   & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}0.00}   & \cellcolor[HTML]{FF0000}No  & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}0.00}   & \cellcolor[HTML]{FF0000}No  & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}0}       & \cellcolor[HTML]{FF0000}No  & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}0}       & \cellcolor[HTML]{FF0000}No  \\ \hline
% NOX       nitric oxides concentration (parts per 10 million)                             & \cellcolor[HTML]{FF0000}\textgreater{}= 0.60  & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}0.54}   & \cellcolor[HTML]{FF0000}No   & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}0.54}   & \cellcolor[HTML]{FF0000}No  & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}0.41}   & \cellcolor[HTML]{FF0000}No  & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}0.453}   & \cellcolor[HTML]{FF0000}No  & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}0.453}   & \cellcolor[HTML]{FF0000}No  \\ \hline
% RM        average number of rooms per dwelling                                           & \cellcolor[HTML]{00FF00}\textgreater{}= 1.41  & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}6.10}   & \cellcolor[HTML]{00FF00}Yes  & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}5.94}   & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}6.82}   & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}6.145}   & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}5.927}   & \cellcolor[HTML]{00FF00}Yes \\ \hline
% AGE       proportion of owner-occupied units built prior to 1940                         & \cellcolor[HTML]{00FF00}\textgreater{}= -0.60 & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}84.50}  & \cellcolor[HTML]{00FF00}Yes  & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}29.30}  & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}40.50}  & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}29.2}    & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}47.2}    & \cellcolor[HTML]{00FF00}Yes \\ \hline
% DIS       weighted distances to five Boston employment centres                           & \cellcolor[HTML]{00FF00}\textgreater{}= 0.85  & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}4.46}   & \cellcolor[HTML]{00FF00}Yes  & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}4.50}   & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}8.32}   & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}7.8148}  & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}6.932}   & \cellcolor[HTML]{00FF00}Yes \\ \hline
% RAD       index of accessibility to radial highways                                      & \cellcolor[HTML]{00FF00}\textgreater{}= 0.37  & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}4.00}   & \cellcolor[HTML]{00FF00}Yes  & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}4.00}   & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}5.00}   & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}8}       & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}8}       & \cellcolor[HTML]{00FF00}Yes \\ \hline
% TAX      full-value property-tax rate per \$10,000                                       & \cellcolor[HTML]{00FF00}\textgreater{}= 0.89  & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}307.00} & \cellcolor[HTML]{00FF00}Yes  & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}307.00} & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}256.00} & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}284}     & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}284}     & \cellcolor[HTML]{00FF00}Yes \\ \hline
% PTRATIO  pupil-teacher ratio by town                                                     & \cellcolor[HTML]{00FF00}\textgreater{}= -0.01 & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}21.00}  & \cellcolor[HTML]{00FF00}Yes  & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}21.00}  & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}15.10}  & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}19.7}    & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}19.7}    & \cellcolor[HTML]{00FF00}Yes \\ \hline
% B        1000(Bk - 0.63)\textasciicircum{}2 where Bk is the proportion of blacks by town & \cellcolor[HTML]{00FF00}\textgreater{}= -1.07 & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}380.02} & \cellcolor[HTML]{00FF00}Yes  & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}386.85} & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}392.90} & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}390.68}  & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}396.9}   & \cellcolor[HTML]{00FF00}Yes \\ \hline
% LSTAT    \% lower status of the population                                               & \cellcolor[HTML]{00FF00}\textgreater{}= -1.17 & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}10.26}  & \cellcolor[HTML]{00FF00}Yes  & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}6.58}   & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}3.95}   & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}6.86}    & \cellcolor[HTML]{00FF00}Yes & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}9.22}    & \cellcolor[HTML]{00FF00}Yes \\ \hline
% \end{tabular}
% \end{table*}

% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage[table,xcdraw]{xcolor}
% % If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


==> tables/rq1table2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[htbp]
\tiny
\centering
  \caption{Applicability of data precondition to detect important features on different datasets}
\begin{tabular}{|l|r|rrlrr|lrr|}
\hline
\rowcolor[HTML]{F3F3F3} 
\cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{F3F3F3} & \multicolumn{5}{c|}{\cellcolor[HTML]{F3F3F3}Data Precondition} & \multicolumn{3}{c|}{\cellcolor[HTML]{F3F3F3}SHAP} \\ \cline{3-10} 
\rowcolor[HTML]{F3F3F3} 
\multirow{-2}{*}{\cellcolor[HTML]{F3F3F3}Dataset} & \multirow{-2}{*}{\cellcolor[HTML]{F3F3F3}Accuracy} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}\# Satisfied} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}\# Violation} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}Least Features} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}Accuracy} & AccDrop & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}Least Features} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}Accuracy} & AccDrop \\ \hline
 & 0.77 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{153} & \multicolumn{1}{l|}{\cellcolor[HTML]{A61C00}Diabetes Pedigree} & \multicolumn{1}{r|}{0.75} & 0.02 & \multicolumn{1}{l|}{\cellcolor[HTML]{0B5394}Insulin} & \multicolumn{1}{r|}{0.77} & 0.00\\ \cline{2-10} 
 & 0.77 & \multicolumn{1}{r|}{74} & \multicolumn{1}{r|}{79} & \multicolumn{1}{l|}{\cellcolor[HTML]{CC0000}Insulin} & \multicolumn{1}{r|}{0.77} & 0.00& \multicolumn{1}{l|}{\cellcolor[HTML]{3D85C6}SkinThickness} & \multicolumn{1}{r|}{0.79} & 0.02 \\ \cline{2-10} 
 & 0.77 & \multicolumn{1}{r|}{103} & \multicolumn{1}{r|}{50} & \multicolumn{1}{l|}{\cellcolor[HTML]{E06666}Skin Thickness} & \multicolumn{1}{r|}{0.79} & -0.02 & \multicolumn{1}{l|}{\cellcolor[HTML]{6FA8DC}\#Pregnancies} & \multicolumn{1}{r|}{0.76} & -0.01 \\ \cline{2-10} 
 & 0.77 & \multicolumn{1}{r|}{136} & \multicolumn{1}{r|}{17} & \multicolumn{1}{l|}{\cellcolor[HTML]{EA9999}\#Pregnancies} & \multicolumn{1}{r|}{0.76} & 0.01 & \multicolumn{1}{l|}{\cellcolor[HTML]{9FC5E8}Blood Pressure} & \multicolumn{1}{r|}{0.77} & 0.00\\ \cline{2-10} 
\multirow{-5}{*}{Pima Diabetes} & 0.77 & \multicolumn{1}{r|}{148} & \multicolumn{1}{r|}{5} & \multicolumn{1}{l|}{\cellcolor[HTML]{F4CCCC}Blood Pressure} & \multicolumn{1}{r|}{0.77} & 0.00& \multicolumn{1}{l|}{\cellcolor[HTML]{CFE2F3}Diabetes Pedigree} & \multicolumn{1}{r|}{0.75} & -0.02 \\ \hline
\cellcolor[HTML]{F3F3F3} & 3.69 & \multicolumn{1}{r|}{95} & \multicolumn{1}{r|}{5} & \multicolumn{1}{l|}{\cellcolor[HTML]{CC0000}CHAS} & \multicolumn{1}{r|}{3.87} & -0.18 & \multicolumn{1}{l|}{\cellcolor[HTML]{0B5394}CHAS} & \multicolumn{1}{r|}{3.87} & 0.18 \\ \cline{2-10} 
\cellcolor[HTML]{F3F3F3} & 3.69 & \multicolumn{1}{r|}{95} & \multicolumn{1}{r|}{5} & \multicolumn{1}{l|}{\cellcolor[HTML]{CC0000}CRIM} & \multicolumn{1}{r|}{3.98} & -0.29 & \multicolumn{1}{l|}{\cellcolor[HTML]{3D85C6}ZN} & \multicolumn{1}{r|}{4.79} & 1.10 \\ \cline{2-10} 
\cellcolor[HTML]{F3F3F3} & 3.69 & \multicolumn{1}{r|}{95} & \multicolumn{1}{r|}{5} & \multicolumn{1}{l|}{\cellcolor[HTML]{CC0000}LSTAT} & \multicolumn{1}{r|}{5.64} & -1.95 & \multicolumn{1}{l|}{\cellcolor[HTML]{6FA8DC}RAD} & \multicolumn{1}{r|}{4.14} & 0.45 \\ \cline{2-10} 
\cellcolor[HTML]{F3F3F3} & 3.69 & \multicolumn{1}{r|}{96} & \multicolumn{1}{r|}{4} & \multicolumn{1}{l|}{\cellcolor[HTML]{E06666}INDUS} & \multicolumn{1}{r|}{3.95} & -0.26 & \multicolumn{1}{l|}{\cellcolor[HTML]{9FC5E8}AGE} & \multicolumn{1}{r|}{3.91} & 0.22 \\ \cline{2-10} 
\multirow{-5}{*}{\cellcolor[HTML]{F3F3F3}Boston Housing} & 3.69 & \multicolumn{1}{r|}{96} & \multicolumn{1}{r|}{4} & \multicolumn{1}{l|}{\cellcolor[HTML]{E06666}AGE} & \multicolumn{1}{r|}{3.91} & -0.22 & \multicolumn{1}{l|}{\cellcolor[HTML]{CFE2F3}INDUS} & \multicolumn{1}{r|}{3.95} & 0.26 \\ \hline
 & 0.89 & \multicolumn{1}{r|}{26} & \multicolumn{1}{r|}{266} & \multicolumn{1}{l|}{\cellcolor[HTML]{990000}Fireplaces} & \multicolumn{1}{r|}{0.84} & 0.05 & \multicolumn{1}{l|}{\cellcolor[HTML]{0B5394}HalfBath} & \multicolumn{1}{r|}{0.88} & -0.01 \\ \cline{2-10} 
 & 0.89 & \multicolumn{1}{r|}{107} & \multicolumn{1}{r|}{185} & \multicolumn{1}{l|}{\cellcolor[HTML]{CC0000}HalfBath} & \multicolumn{1}{r|}{0.88} & 0.01 & \multicolumn{1}{l|}{\cellcolor[HTML]{3D85C6}BedroomAbvGr} & \multicolumn{1}{r|}{0.88} & -0.01 \\ \cline{2-10} 
 & 0.89 & \multicolumn{1}{r|}{161} & \multicolumn{1}{r|}{131} & \multicolumn{1}{l|}{\cellcolor[HTML]{E06666}FullBath} & \multicolumn{1}{r|}{0.77} & 0.12 & \multicolumn{1}{l|}{\cellcolor[HTML]{6FA8DC}OverallQual} & \multicolumn{1}{r|}{0.9} & 0.01 \\ \cline{2-10} 
 & 0.89 & \multicolumn{1}{r|}{275} & \multicolumn{1}{r|}{17} & \multicolumn{1}{l|}{\cellcolor[HTML]{EA9999}GarageArea} & \multicolumn{1}{r|}{0.93} & -0.04 & \multicolumn{1}{l|}{\cellcolor[HTML]{9FC5E8}TotRmsAbvGrd} & \multicolumn{1}{r|}{0.93} & 0.04 \\ \cline{2-10} 
\multirow{-5}{*}{House Price} & 0.89 & \multicolumn{1}{r|}{287} & \multicolumn{1}{r|}{5} & \multicolumn{1}{l|}{\cellcolor[HTML]{F4CCCC}TotalBsmtSF} & \multicolumn{1}{r|}{0.92} & -0.03 & \multicolumn{1}{l|}{\cellcolor[HTML]{CFE2F3}FullBath} & \multicolumn{1}{r|}{0.77} & -0.12 \\ \hline
\cellcolor[HTML]{F3F3F3} & 0.97 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{418} & \multicolumn{1}{l|}{\cellcolor[HTML]{980000}Pclass} & \multicolumn{1}{r|}{0.96} & 0.01 & \multicolumn{1}{l|}{\cellcolor[HTML]{0B5394}Others} & \multicolumn{1}{r|}{0.96} & -0.01 \\ \cline{2-10} 
\cellcolor[HTML]{F3F3F3} & 0.97 & \multicolumn{1}{r|}{6} & \multicolumn{1}{r|}{412} & \multicolumn{1}{l|}{\cellcolor[HTML]{CC0000}Family} & \multicolumn{1}{r|}{0.95} & 0.02 & \multicolumn{1}{l|}{\cellcolor[HTML]{3D85C6}Pclass} & \multicolumn{1}{r|}{0.96} & -0.01 \\ \cline{2-10} 
\cellcolor[HTML]{F3F3F3} & 0.97 & \multicolumn{1}{r|}{30} & \multicolumn{1}{r|}{388} & \multicolumn{1}{l|}{\cellcolor[HTML]{E06666}Ticket\_C} & \multicolumn{1}{r|}{0.96} & 0.01 & \multicolumn{1}{l|}{\cellcolor[HTML]{6FA8DC}Age-bin} & \multicolumn{1}{r|}{0.97} & 0.00\\ \cline{2-10} 
\cellcolor[HTML]{F3F3F3} & 0.97 & \multicolumn{1}{r|}{33} & \multicolumn{1}{r|}{385} & \multicolumn{1}{l|}{\cellcolor[HTML]{CC0000}Ticket\_P} & \multicolumn{1}{r|}{0.96} & 0.01 & \multicolumn{1}{l|}{\cellcolor[HTML]{9FC5E8}Fare-bin} & \multicolumn{1}{r|}{0.96} & -0.01 \\ \cline{2-10} 
\multirow{-5}{*}{\cellcolor[HTML]{F3F3F3}Titanic} & 0.97 & \multicolumn{1}{r|}{73} & \multicolumn{1}{r|}{345} & \multicolumn{1}{l|}{\cellcolor[HTML]{E6B8AF}Others} & \multicolumn{1}{r|}{0.96} & 0.01 & \multicolumn{1}{l|}{\cellcolor[HTML]{CFE2F3}Sex} & \multicolumn{1}{r|}{0.97} & 0.00\\ \hline
 & 0.81 & \multicolumn{1}{r|}{14} & \multicolumn{1}{r|}{2102} & \multicolumn{1}{l|}{\cellcolor[HTML]{990000}job\_unknown} & \multicolumn{1}{r|}{0.81} & 0.00& \multicolumn{1}{l|}{\cellcolor[HTML]{0B5394}marital\_single} & \multicolumn{1}{r|}{0.82} & 0.01 \\ \cline{2-10} 
 & 0.81 & \multicolumn{1}{r|}{68} & \multicolumn{1}{r|}{2048} & \multicolumn{1}{l|}{\cellcolor[HTML]{CC0000}job\_entrepreneur} & \multicolumn{1}{r|}{0.81} & 0.00& \multicolumn{1}{l|}{\cellcolor[HTML]{3D85C6}housing\_yes} & \multicolumn{1}{r|}{0.82} & 0.01 \\ \cline{2-10} 
 & 0.81 & \multicolumn{1}{r|}{170} & \multicolumn{1}{r|}{1946} & \multicolumn{1}{l|}{\cellcolor[HTML]{E06666}contact\_telephone} & \multicolumn{1}{r|}{0.82} & -0.01 & \multicolumn{1}{l|}{\cellcolor[HTML]{6FA8DC}poutcome} & \multicolumn{1}{r|}{0.82} & 0.01 \\ \cline{2-10} 
 & 0.81 & \multicolumn{1}{r|}{186} & \multicolumn{1}{r|}{1930} & \multicolumn{1}{l|}{\cellcolor[HTML]{EA9999}job\_services} & \multicolumn{1}{r|}{0.82} & -0.01 & \multicolumn{1}{l|}{\cellcolor[HTML]{9FC5E8}day} & \multicolumn{1}{r|}{0.81} & 0.00\\ \cline{2-10} 
\multirow{-5}{*}{Bank Customer} & 0.81 & \multicolumn{1}{r|}{290} & \multicolumn{1}{r|}{1826} & \multicolumn{1}{l|}{\cellcolor[HTML]{F4CCCC}loan\_yes} & \multicolumn{1}{r|}{0.81} & 0.00& \multicolumn{1}{l|}{\cellcolor[HTML]{CFE2F3}education} & \multicolumn{1}{r|}{0.81} & 0.00\\ \hline
\end{tabular}
  \label{tab:rq1FeatureImportance}%
  \footnotesize
     
  { * Here, feature importance interpretation by our approach: (\least{least} important feature to \most{more} important features) and SHAP approach: (\leastB{least} important feature to \mostB{more} important features).}
\end{table*}








% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage[table,xcdraw]{xcolor}
% % If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table*}[htbp]
% \tiny
% \centering
%   \caption{Applicability of data precondition to detect important features on different datasets}
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage[table,xcdraw]{xcolor}
% % If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{tabular}{|l|l|rr|l|rr|}
% \hline
% \rowcolor[HTML]{F3F3F3} 
% \multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}} & \cellcolor[HTML]{F3F3F3} & \multicolumn{2}{c|}{\cellcolor[HTML]{F3F3F3}Model \#1} & \cellcolor[HTML]{F3F3F3} & \multicolumn{2}{c|}{\cellcolor[HTML]{F3F3F3}Model \#4} \\ \cline{3-4} \cline{6-7} 
% \rowcolor[HTML]{F3F3F3} 
% \multicolumn{1}{|c|}{\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}Dataset}} & \multirow{-2}{*}{\cellcolor[HTML]{F3F3F3}Features} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}\# Satisfied} & \# Violation & \multirow{-2}{*}{\cellcolor[HTML]{F3F3F3}Features} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}\# Satisfied} & \# Violation \\ \hline
%  & \cellcolor[HTML]{EA9999}\#Pregnancies & \multicolumn{1}{r|}{136} & 17 & \cellcolor[HTML]{EA9999}\#Pregnancies & \multicolumn{1}{r|}{136} & 17 \\ \cline{2-7} 
%  & Glucose & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}153} & \cellcolor[HTML]{D9EAD3}0.00& Glucose & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}153} & \cellcolor[HTML]{D9EAD3}0.00\\ \cline{2-7} 
%  & \cellcolor[HTML]{F4CCCC}Blood Pressure & \multicolumn{1}{r|}{148} & 5 & \cellcolor[HTML]{F4CCCC}Blood Pressure & \multicolumn{1}{r|}{148} & 5 \\ \cline{2-7} 
%  & \cellcolor[HTML]{E06666}Skin Thickness & \multicolumn{1}{r|}{103} & 50.00& \cellcolor[HTML]{E06666}Skin Thickness & \multicolumn{1}{r|}{103} & 50.00\\ \cline{2-7} 
%  & \cellcolor[HTML]{CC0000}Insulin & \multicolumn{1}{r|}{74} & 79 & \cellcolor[HTML]{CC0000}Insulin & \multicolumn{1}{r|}{74} & 79 \\ \cline{2-7} 
%  & BMI & \multicolumn{1}{r|}{151} & 2 & BMI & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}153} & \cellcolor[HTML]{D9EAD3}0.00\\ \cline{2-7} 
%  & \cellcolor[HTML]{990000}Diabetes Pedigree function & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}153 & Diabetes Pedigree function & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}153} & \cellcolor[HTML]{D9EAD3}0.00\\ \cline{2-7} 
% \multirow{-8}{*}{Pima Diabetes} & Age & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}153} & \cellcolor[HTML]{D9EAD3}0.00& Age & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}153} & \cellcolor[HTML]{D9EAD3}0.00\\ \hline
% \cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{CC0000}CRIM & \multicolumn{1}{r|}{95} & 5 & \cellcolor[HTML]{CC0000}CRIM & \multicolumn{1}{r|}{95} & 5 \\ \cline{2-7} 
% \cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{F3F3F3}ZN & \multicolumn{1}{r|}{98} & 2 & \cellcolor[HTML]{F3F3F3}ZN & \multicolumn{1}{r|}{98} & 2 \\ \cline{2-7} 
% \cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{E06666}INDUS & \multicolumn{1}{r|}{96} & 4 & \cellcolor[HTML]{E06666}INDUS & \multicolumn{1}{r|}{96} & 4 \\ \cline{2-7} 
% \cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{CC0000}CHAS & \multicolumn{1}{r|}{95} & 5 & \cellcolor[HTML]{CC0000}CHAS & \multicolumn{1}{r|}{95} & 5 \\ \cline{2-7} 
% \rowcolor[HTML]{D9EAD3} 
% \cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{F3F3F3}NOX & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & 0.00& \cellcolor[HTML]{F3F3F3}NOX & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & 0.00\\ \cline{2-7} 
% \rowcolor[HTML]{D9EAD3} 
% \cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{F3F3F3}RM & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & 0.00& \cellcolor[HTML]{F3F3F3}RM & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & 0.00\\ \cline{2-7} 
% \rowcolor[HTML]{F3F3F3} 
% \cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{E06666}AGE & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}96} & 4 & \cellcolor[HTML]{E06666}AGE & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}96} & 4 \\ \cline{2-7} 
% \rowcolor[HTML]{D9EAD3} 
% \cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{F3F3F3}DIS & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & 0.00& \cellcolor[HTML]{F3F3F3}DIS & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & 0.00\\ \cline{2-7} 
% \rowcolor[HTML]{D9EAD3} 
% \cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{F3F3F3}RAD & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & 0.00& \cellcolor[HTML]{F3F3F3}RAD & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & 0.00\\ \cline{2-7} 
% \rowcolor[HTML]{D9EAD3} 
% \cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{F3F3F3}TAX & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & 0.00& \cellcolor[HTML]{F3F3F3}TAX & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & 0.00\\ \cline{2-7} 
% \rowcolor[HTML]{D9EAD3} 
% \cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{F3F3F3}PTRATIO & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & 0.00& \cellcolor[HTML]{F3F3F3}PTRATIO & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & 0.00\\ \cline{2-7} 
% \rowcolor[HTML]{D9EAD3} 
% \cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{F3F3F3}B & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & 0.00& \cellcolor[HTML]{F3F3F3}B & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & 0.00\\ \cline{2-7} 
% \multirow{-13}{*}{\cellcolor[HTML]{F3F3F3}Boston Housing} & \cellcolor[HTML]{CC0000}LSTAT & \multicolumn{1}{r|}{95} & 5 & \cellcolor[HTML]{CC0000}LSTAT & \multicolumn{1}{r|}{95} & 5 \\ \hline
%  & LotArea & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}292} & \cellcolor[HTML]{D9EAD3}0.00& LotArea & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}292} & \cellcolor[HTML]{D9EAD3}0.00\\ \cline{2-7} 
%  & OverallQual & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}292} & \cellcolor[HTML]{D9EAD3}0.00& OverallQual & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}292} & \cellcolor[HTML]{D9EAD3}0.00\\ \cline{2-7} 
%  & OverallCond & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}292} & \cellcolor[HTML]{D9EAD3}0.00& OverallCond & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}292} & \cellcolor[HTML]{D9EAD3}0.00\\ \cline{2-7} 
%  & \cellcolor[HTML]{F4CCCC}TotalBsmtSF & \multicolumn{1}{r|}{287} & 5 & \cellcolor[HTML]{EA9999}TotalBsmtSF & \multicolumn{1}{r|}{287} & 5 \\ \cline{2-7} 
%  & \cellcolor[HTML]{E06666}FullBath & \multicolumn{1}{r|}{161} & 131 & FullBath & \multicolumn{1}{r|}{289} & 3 \\ \cline{2-7} 
%  & \cellcolor[HTML]{CC0000}HalfBath & \multicolumn{1}{r|}{107} & 185 & \cellcolor[HTML]{990000}HalfBath & \multicolumn{1}{r|}{107} & 185 \\ \cline{2-7} 
%  & BedroomAbvGr & \multicolumn{1}{r|}{289} & 3 & \cellcolor[HTML]{F4CCCC}BedroomAbvGr & \multicolumn{1}{r|}{289} & 3 \\ \cline{2-7} 
%  & TotRmsAbvGrd & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}292} & \cellcolor[HTML]{D9EAD3}0.00& TotRmsAbvGrd & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}292} & \cellcolor[HTML]{D9EAD3}0.00\\ \cline{2-7} 
%  & \cellcolor[HTML]{990000}Fireplaces & \multicolumn{1}{r|}{26} & 266 & \cellcolor[HTML]{CC0000}Fireplaces & \multicolumn{1}{r|}{156} & 136 \\ \cline{2-7} 
% \multirow{-10}{*}{House Price} & \cellcolor[HTML]{EA9999}GarageArea & \multicolumn{1}{r|}{275} & 17 & \cellcolor[HTML]{E06666}GarageArea & \multicolumn{1}{r|}{275} & 17 \\ \hline
% \rowcolor[HTML]{F4CCCC} 
% \cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{980000}Pclass & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & 418 & \cellcolor[HTML]{980000}Pclass & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & 418 \\ \cline{2-7} 
% \cellcolor[HTML]{F3F3F3} & Sex & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0.00& Sex & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0.00\\ \cline{2-7} 
% \cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{F3F3F3}Master & \multicolumn{1}{r|}{152} & 266 & \cellcolor[HTML]{F3F3F3}Master & \multicolumn{1}{r|}{152} & 266 \\ \cline{2-7} 
% \cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{F3F3F3}Miss & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0.00& \cellcolor[HTML]{F3F3F3}Miss & \multicolumn{1}{r|}{21} & 397 \\ \cline{2-7} 
% \cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{F3F3F3}Mr & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0.00& \cellcolor[HTML]{F3F3F3}Mr & \multicolumn{1}{r|}{78} & 340.00\\ \cline{2-7} 
% \cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{F3F3F3}Mrs & \multicolumn{1}{r|}{240} & 178 & \cellcolor[HTML]{F3F3F3}Mrs & \multicolumn{1}{r|}{240} & 178 \\ \cline{2-7} 
% \cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{E6B8AF}Others & \multicolumn{1}{r|}{73} & 345 & \cellcolor[HTML]{E6B8AF}Others & \multicolumn{1}{r|}{73} & 345 \\ \cline{2-7} 
% \cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{CC0000}Family & \multicolumn{1}{r|}{6} & 412 & \cellcolor[HTML]{CC0000}Family & \multicolumn{1}{r|}{6} & 412 \\ \cline{2-7} 
% \cellcolor[HTML]{F3F3F3} & Fare-bin & \multicolumn{1}{r|}{398} & 20.00& Fare-bin & \multicolumn{1}{r|}{398} & 20.00\\ \cline{2-7} 
% \rowcolor[HTML]{D9EAD3} 
% \cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{F3F3F3}Age-bin & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & 0.00& \cellcolor[HTML]{F3F3F3}Age-bin & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & 0.00\\ \cline{2-7} 
% \rowcolor[HTML]{D9EAD3} 
% \cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{F3F3F3}Ticket\_1 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & 0.00& \cellcolor[HTML]{F3F3F3}Ticket\_1 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & 0.00\\ \cline{2-7} 
% \rowcolor[HTML]{D9EAD3} 
% \cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{F3F3F3}Ticket\_2 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & 0.00& \cellcolor[HTML]{F3F3F3}Ticket\_2 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & 0.00\\ \cline{2-7} 
% \cellcolor[HTML]{F3F3F3} & Ticket\_3 & \multicolumn{1}{r|}{95} & 323 & Ticket\_3 & \multicolumn{1}{r|}{95} & 323 \\ \cline{2-7} 
% \cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{F3F3F3}Ticket\_4 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0.00& \cellcolor[HTML]{F3F3F3}Ticket\_4 & \multicolumn{1}{r|}{35} & 383 \\ \cline{2-7} 
% \cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{E06666}Ticket\_C & \multicolumn{1}{r|}{30} & 388 & \cellcolor[HTML]{E06666}Ticket\_C & \multicolumn{1}{r|}{30} & 388 \\ \cline{2-7} 
% \cellcolor[HTML]{F3F3F3} & \cellcolor[HTML]{CC0000}Ticket\_P & \multicolumn{1}{r|}{33} & 385 & \cellcolor[HTML]{CC0000}Ticket\_P & \multicolumn{1}{r|}{33} & 385 \\ \cline{2-7} 
% \multirow{-17}{*}{\cellcolor[HTML]{F3F3F3}Titanic} & \cellcolor[HTML]{F3F3F3}Ticket\_S & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0.00& \cellcolor[HTML]{F3F3F3}Ticket\_S & \multicolumn{1}{r|}{33} & 385 \\ \hline

% \end{tabular}
%   \label{tab:rq1FeatureImportance}%
%   \footnotesize
     
%   { * Here, feature importance interpretation: (\least{least} important feature to \most{more} important features).}
% \end{table*}


==> tables/rq1table3.tex <==
\begin{table*}[htbp]
\footnotesize
  \centering
  \caption{Feature removal experiment with PIMA dataset}
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{tabular}{|l|rr|}
\hline
                                                                      & \multicolumn{2}{r|}{\textbf{ALL test data examples (20\%)}}                                                                                 \\ \hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Features}                                                     & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}\textbf{Average Loss}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{Average Accuracy}} \\ \hline
ALL                                                                   & \multicolumn{1}{r|}{\textbf{0.4944}}                               & \textbf{76.69\%}                                                       \\ \hline
ALL - \{Diabetes Pedigree function\}                                  & \multicolumn{1}{r|}{0.5155}                                        & 74.60\%                                                                \\ \hline
ALL - \{\#Pregnancies\}                                               & \multicolumn{1}{r|}{0.5343}                                        & 72.78\%                                                                \\ \hline
ALL - \{Insulin\}                                                     & \multicolumn{1}{r|}{0.4875}                                        & 76.95\%                                                                \\ \hline
\rowcolor[HTML]{D9EAD3} 
\textbf{ALL - \{Diabetes Pedigree function, \#Pregnancies, Insulin\}} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}\textbf{0.5049}}       & \textbf{76.43\%}                                                       \\ \hline
\end{tabular}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[htbp]
  \centering
  \caption{Feature removal experiment with Titanic dataset}
\begin{tabular}{llllllllllllllllllllll}
\cline{2-3}
\multicolumn{1}{l|}{}                                           & \multicolumn{2}{r|}
{\textbf{After Removing each features}}                                                                                  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-3}
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}\textbf{Features}} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}\textbf{Average Loss}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{Average Accuracy}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-3}
\multicolumn{1}{|l|}{ALL}                                       & \multicolumn{1}{r|}{\textbf{0.397}}                                & \multicolumn{1}{r|}{\textbf{83.19\%}}                                  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-3}
\multicolumn{1}{|l|}{ALL - \{Master\}}                          & \multicolumn{1}{r|}{0.061}                                         & \multicolumn{1}{r|}{97.56\%}                                           &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-3}
\multicolumn{1}{|l|}{ALL - \{Ticket\_1\}}                       & \multicolumn{1}{r|}{0.059}                                         & \multicolumn{1}{r|}{97.50\%}                                           &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-3}
\multicolumn{1}{|l|}{ALL - \{Ticket\_4\}}                       & \multicolumn{1}{r|}{0.071}                                         & \multicolumn{1}{r|}{96.67\%}                                           &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-3}
\multicolumn{1}{|l|}{ALL - \{Ticket\_C\}}                       & \multicolumn{1}{r|}{0.072}                                         & \multicolumn{1}{r|}{96.99\%}                                           &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-3}
\multicolumn{1}{|l|}{ALL - \{Ticket\_3\}}                       & \multicolumn{1}{r|}{0.069}                                         & \multicolumn{1}{r|}{96.85\%}                                           &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-3}
\multicolumn{1}{|l|}{ALL - \{Gender\}}                          & \multicolumn{1}{r|}{0.065}                                         & \multicolumn{1}{r|}{97.26\%}             \\
\cline{1-3}
\end{tabular}
\end{table*}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[htbp]
\centering
  \caption{Feature removal experiment with house price prediction dataset}
\begin{tabular}{|l|rr|}
\hline
                                   & \multicolumn{2}{l|}{\cellcolor[HTML]{EFEFEF}ALL test data examples (20\%)}                                                             \\ \cline{2-3} 
\multirow{-2}{*}{Features}         & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{Average Loss}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{Average MAE}} \\ \hline
\textbf{ALL}                       & \multicolumn{1}{r|}{\textbf{30.62}}                                & \textbf{4}                                                        \\ \hline
ALL - \{CRIM\}                     & \multicolumn{1}{r|}{29.44}                                         & 3.76                                                              \\ \hline
ALL - \{CHAS\}                     & \multicolumn{1}{r|}{31.29}                                         & 3.92                                                              \\ \hline
ALL - \{NOX\}                      & \multicolumn{1}{r|}{31.77}                                         & 4.12                                                              \\ \hline
\rowcolor[HTML]{D9EAD3} 
\textbf{ALL - \{CRIM, CHAS, NOX\}} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}\textbf{28.99}}        & \textbf{3.9}                                                      \\ \hline
\end{tabular}
\end{table*}

==> tables/rq2table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[htbp]
\tiny
\centering
\caption{Out-of-distribution feature detection using data precondition violation}
\label{tab:missval}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|rrrr|rrrr|rrrr|rrrr|}
\hline
\rowcolor[HTML]{D9D9D9} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9} & \multicolumn{4}{c|}{\cellcolor[HTML]{D9D9D9}Model \#1} & \multicolumn{4}{c|}{\cellcolor[HTML]{D9D9D9}Model \#2} & \multicolumn{4}{c|}{\cellcolor[HTML]{D9D9D9}Model \#3} & \multicolumn{4}{c|}{\cellcolor[HTML]{D9D9D9}Model \#4} \\ \cline{3-18} 
\rowcolor[HTML]{D9D9D9} 
\multirow{-2}{*}{\cellcolor[HTML]{D9D9D9}Dataset} & \multirow{-2}{*}{\cellcolor[HTML]{D9D9D9}Features} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}OOD} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}MD} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}\#S} & \#V & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}OOD} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}MD} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}\#S} & \#V & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}OOD} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}MD} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}\#S} & \#V & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}OOD} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}MD} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}\#S} & \#V \\ \hline
 & \#Pregnancies & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}17} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{136} & 17 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}153} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}153 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}108} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{45} & 108 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}17} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{136} & 17 \\ \cline{2-18} 
 & Glucose & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}153} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}153} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}153 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}153} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}153 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}153} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
 & Blood Pressure & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}5} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{148} & 5 & \multicolumn{1}{r|}{148} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{5} & 148 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}153} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}153 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}5} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{148} & 5 \\ \cline{2-18} 
 & Skin Thickness & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}50} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{103} & 50 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}153} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}153 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}103} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{50} & 103 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}50} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{103} & 50 \\ \cline{2-18} 
 & Insulin & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}79} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{74} & 79 & \multicolumn{1}{r|}{74} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{79} & 74 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}153} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}153 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}79} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{74} & 79 \\ \cline{2-18} 
 & BMI & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{151} & 2 & \multicolumn{1}{r|}{151} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2} & 151 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}153} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}153 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}153} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
 & Pedigree & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}153} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}153 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}153} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}153 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}43} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{110} & 43 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}153} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
\multirow{-8}{*}{Pima Diabetes} & Age & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}153} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}153} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}153 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}153} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}153 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}153} & \cellcolor[HTML]{D9EAD3}0 \\ \hline
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}CRIM & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}5} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}95} & \cellcolor[HTML]{F3F3F3}5 & \multicolumn{1}{r|}{95} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}5} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{95} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}5} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}5} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}95} & \cellcolor[HTML]{F3F3F3}5 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}ZN & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}2} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}98} & \cellcolor[HTML]{F3F3F3}2 & \multicolumn{1}{r|}{98} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}2} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{98} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}2} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}2} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}98} & \cellcolor[HTML]{F3F3F3}2 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}INDUS & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}4} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}96} & \cellcolor[HTML]{F3F3F3}4 & \multicolumn{1}{r|}{96} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}4} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{96} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}4} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}4} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}96} & \cellcolor[HTML]{F3F3F3}4 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}CHAS & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}5} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}95} & \cellcolor[HTML]{F3F3F3}5 & \multicolumn{1}{r|}{95} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}5} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{95} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}5} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}5} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}95} & \cellcolor[HTML]{F3F3F3}5 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}NOX & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}RM & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}AGE & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}4} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}96} & \cellcolor[HTML]{F3F3F3}4 & \multicolumn{1}{r|}{96} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}4} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}96} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}4} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}4} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}96} & \cellcolor[HTML]{F3F3F3}4 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}DIS & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}RAD & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}TAX & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}PTRATIO & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}B & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
\multirow{-13}{*}{\cellcolor[HTML]{D9D9D9}BostonHousing} & \cellcolor[HTML]{D9D9D9}LSTAT & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}5} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}95} & \cellcolor[HTML]{F3F3F3}5 & \multicolumn{1}{r|}{95} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}5} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{95} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}5} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}5} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}95} & \cellcolor[HTML]{F3F3F3}5 \\ \hline
 & LotArea & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}292} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}292} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}292 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}292} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}292 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}292} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
 & OverallQual & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}292} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}292} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}292 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}292} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}292 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}292} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
 & OverallCond & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}292} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}292} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}292 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}292} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}292 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}292} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
 & TotalBsmtSF & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}5} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{287} & 5 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}287} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{5} & 287 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}292} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}292 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}5} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{287} & 5 \\ \cline{2-18} 
 & FullBath & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}131} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{161} & 131 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}289} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{3} & 289 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}289} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{3} & 289 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}3} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{289} & 3 \\ \cline{2-18} 
 & HalfBath & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}185} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{107} & 185 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}107} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{185} & 107 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}107} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{185} & 107 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}185} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{107} & 185 \\ \cline{2-18} 
 & BedroomAbvGr & \multicolumn{1}{r|}{3} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{289} & 3 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}289} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{3} & 289 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}292} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}292 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}3} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{289} & 3 \\ \cline{2-18} 
 & TotRmsAbvGrd & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}292} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}292} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}292 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}292} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}292 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}292} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
 & Fireplaces & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}266} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{26} & 266 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}156} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{136} & 156 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}156} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{136} & 156 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}136} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{156} & 136 \\ \cline{2-18} 
\multirow{-10}{*}{HousePricePredictionData} & GarageArea & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}17} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{275} & 17 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}275} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{17} & 275 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}292} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}292 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}17} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{275} & 17 \\ \hline
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Pclass & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{CFE2F3}418} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}418} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}418} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}418} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Sex & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}218} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{200} & 218 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Master & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}266} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{152} & 266 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}266} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{152} & 266 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Miss & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}21} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{397} & 21 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}397} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{21} & 397 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Mr & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}340} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{78} & 340 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Mrs & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}178} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{240} & 178 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}240} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{178} & 240 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}240} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{178} & 240 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}178} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{240} & 178 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Others & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}345} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{73} & 345 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}73} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{345} & 73 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}345} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{73} & 345 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Family & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}412} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{6} & 412 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}6} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{412} & 6 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}6} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{412} & 6 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}412} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{6} & 412 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Fare-bin & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}20} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{398} & 20 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}145} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{273} & 145 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}398} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{20} & 398 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}20} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{398} & 20 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Age-bin & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{E6B8AF}0} & \cellcolor[HTML]{E6B8AF}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Ticket\_1 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{E6B8AF}0} & \cellcolor[HTML]{E6B8AF}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Ticket\_2 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}64} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{354} & 64 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Ticket\_3 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}323} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{95} & 323 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}323} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{95} & 323 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Ticket\_4 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}383} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{35} & 383 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Ticket\_C & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}388} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{30} & 388 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{E6B8AF}0} & \cellcolor[HTML]{E6B8AF}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}388} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{30} & 388 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Ticket\_P & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}385} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{33} & 385 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{E6B8AF}0} & \cellcolor[HTML]{E6B8AF}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}33} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{385} & 33 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}385} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{33} & 385 \\ \cline{2-18} 
\multirow{-17}{*}{\cellcolor[HTML]{D9D9D9}Titanic} & \cellcolor[HTML]{D9D9D9}Ticket\_S & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{E6B8AF}0} & \cellcolor[HTML]{E6B8AF}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}33} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{385} & 33 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}385} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{33} & 385 \\ \hline
 & age & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
 & education & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}95} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2021} & 95 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2021} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{95} & 2021 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}95} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2021} & 95 \\ \cline{2-18} 
 & balance & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}294} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1822} & 294 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1971} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{145} & 1971 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1822} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{294} & 1822 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}145} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1971} & 145 \\ \cline{2-18} 
 & day & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
 & month & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
 & duration & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
 & campaign & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
 & pdays & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1602} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{514} & 1602 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}514} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1602} & 514 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}514} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1602} & 514 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1602} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{514} & 1602 \\ \cline{2-18} 
 & previous & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1602} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{514} & 1602 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}514} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1602} & 514 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}514} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1602} & 514 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1602} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{514} & 1602 \\ \cline{2-18} 
 & poutcome & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1603} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{513} & 1603 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2116} & 0 \\ \cline{2-18} 
 & job\_blue & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1734} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{382} & 1734 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}382} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1734} & 382 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1734} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{382} & 1734 \\ \cline{2-18} 
 & job\_entrepren & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2048} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{68} & 2048 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}68} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2048} & 68 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2048} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{68} & 2048 \\ \cline{2-18} 
 & job\_housemaid & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2071} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{45} & 2071 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}45} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2071} & 45 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}45} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2071} & 45 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
 & job\_manage & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1641} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{475} & 1641 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}475} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{164} & 475 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
 & job\_retired & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1971} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{145} & 1971 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}145} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1971} & 145 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
 & job\_self & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2041} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{75} & 2041 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}75} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2041} & 75 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
 & job\_services & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1930} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{186} & 1930 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}186} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1930} & 186 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}186} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1930} & 186 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1930} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{186} & 1930 \\ \cline{2-18} 
 & job\_student & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2046} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{70} & 2046 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}70} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2046} & 70 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}70} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2046} & 70 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
 & job\_technician & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1781} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{335} & 1781 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}335} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1781} & 335 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}335} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1781} & 335 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1781} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{335} & 1781 \\ \cline{2-18} 
 & job\_unemployed & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2049} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{67} & 2049 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}67} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2049} & 67 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}67} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2049} & 67 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
 & job\_unknown & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2102} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{14} & 2102 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}14} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2102} & 14 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}14} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2102} & 14 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2102} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{14} & 2102 \\ \cline{2-18} 
 & marital\_married & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}916} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1200} & 916 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{916} & 1200 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}916} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1200} & 916 \\ \cline{2-18} 
 & marital\_single & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1443} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{673} & 1443 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}673} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1443} & 673 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}673} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1443} & 673 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
 & default\_yes & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2079} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{37} & 2079 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}37} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2079} & 37 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
 & housing\_yes & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1107} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1009} & 1107 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1009} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1107} & 1009 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1009} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1107} & 1009 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1107} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1009} & 1107 \\ \cline{2-18} 
 & loan\_yes & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1826} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{290} & 1826 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}290} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1826} & 290 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1826} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{290} & 1826 \\ \cline{2-18} 
 & telephone & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1946} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{170} & 1946 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}170} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1946} & 170 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}170} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1946} & 170 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1946} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{170} & 1946 \\ \cline{2-18} 
\multirow{-28}{*}{BankCustomer} & unknown & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1650} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{466} & 1650 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}466} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1650} & 466 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}466} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1650} & 466 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1650} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{466} & 1650 \\ \hline
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Age & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}187} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{13} & 187 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}200 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}192} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{8} & 192 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}194} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{6} & 194 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Job & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}44} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{156} & 44 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}156} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{44} & 156 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}195} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{5} & 195 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}171} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{29} & 171 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Credit amount & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}154} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{46} & 154 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}39} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{161} & 39 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}166} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{34} & 166 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}196} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{4} & 196 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Duration & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}183} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{17} & 183 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}48} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{152} & 48 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}142} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{58} & 142 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}198} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2} & 198 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Sex\_female & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}145} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{55} & 145 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}55} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{145} & 55 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}200 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & 200 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Sex\_male & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}55} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{145} & 55 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}145} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{55} & 145 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}200 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & 200 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Housing\_free & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}182} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{18} & 182 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}18} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{182} & 18 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}18} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}182} & \cellcolor[HTML]{F3F3F3}18 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}182} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{18} & 182 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Housing\_own & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}57} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{143} & 57 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}143} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{57} & 143 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}200 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & 200 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Housing\_rent & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}161} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{39} & 161 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}39} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{161} & 39 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}39} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{161} & 39 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}161} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{39} & 161 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}SA\_little & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}73} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{127} & 73 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}127} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{73} & 127 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}127} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{73} & 127 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & 200 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}SA\_moderate & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}186} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{14} & 186 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}14} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{186} & 14 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}14} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{186} & 14 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}186} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{14} & 186 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}SA\_quite rich & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}188} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{12} & 188 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}200 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}12} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{188} & 12 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}188} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{12} & 188 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}SA\_rich & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}194} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{6} & 194 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}6} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{194} & 6 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}200 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}194} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{6} & 194 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}CA\_little & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}135} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{65} & 135 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}65} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{135} & 65 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}65} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{135} & 65 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & 200 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}CA\_moderate & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}157} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{43} & 157 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}43} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{157} & 43 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}43} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{157} & 43 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}157} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{43} & 157 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}CA\_rich & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}192} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{8} & 192 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}8} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{192} & 8 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}8} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{192} & 8 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}192} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{8} & 192 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}P\_business & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}180} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{20} & 180 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}20} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{180} & 20 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}20} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{180} & 20 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & 200 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}P\_car & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}128} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{72} & 128 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}72} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{128} & 72 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}72} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{128} & 72 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & 200 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}P\_appliances & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}197} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{3} & 197 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}3} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{197} & 3 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}3} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{197} & 3 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & 200 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}P\_education & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}194} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{6} & 194 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}6} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{194} & 6 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}6} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{194} & 6 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & 200 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}P\_furniture & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}163} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{37} & 163 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}37} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{163} & 37 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}200 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & 200 \\ \cline{2-18} 
\cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}P\_radio/TV & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}143} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{57} & 143 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}57} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{143} & 57 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}57} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{143} & 57 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}143} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{57} & 143 \\ \cline{2-18} 
\multirow{-23}{*}{\cellcolor[HTML]{D9D9D9}GermanCredit} & \cellcolor[HTML]{D9D9D9}P\_repairs & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}197} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{3} & 197 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}3} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{197} & 3 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}200 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}197} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{3} & 197 \\ \hline
\end{tabular}%
}
  \tiny
     
  { * Here, \violet{cells} represent total out-of-distribution (\# OOD) values detected for a feature, \cyan{cells} represent total missing (\# Miss) values for that particular feature,  \red{cells} denote where data precondition is violated for all test data examples  and \green{cells} indicate where data precondition is satisfied for all test data examples.}
  \label{tab:rq2table}
\end{table*}

% \begin{table*}[htbp]
% \tiny
% \centering
% \caption{Out-of-distribution feature detection using data precondition violation}
% \label{tab:missval}
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage[table,xcdraw]{xcolor}
% % If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{tabular}{|l|l|rrrr|rrrr|rrrr|rrrr|}
% \hline
% \rowcolor[HTML]{D9D9D9} 
% \multicolumn{1}{|c|}{\cellcolor[HTML]{D9D9D9}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}} & \multicolumn{4}{c|}{\cellcolor[HTML]{D9D9D9}Model \#1} & \multicolumn{4}{c|}{\cellcolor[HTML]{D9D9D9}Model \#2} & \multicolumn{4}{c|}{\cellcolor[HTML]{D9D9D9}Model \#3} & \multicolumn{4}{c|}{\cellcolor[HTML]{D9D9D9}Model \#4} \\ \cline{3-18} 
% \rowcolor[HTML]{D9D9D9} 
% \multicolumn{1}{|c|}{\multirow{-2}{*}{\cellcolor[HTML]{D9D9D9}Dataset}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{D9D9D9}Features}} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}\# OOD} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}\# Miss} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}\# Sat} & \# Viol & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}\# OOD} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}\# Miss} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}\# Sat} & \# Viol & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}\# OOD} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}\# Miss} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}\# Sat} & \# Viol & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}\# OOD} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}\# Miss} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}\# Sat} & \# Viol \\ \hline
%  & \#Pregnancies & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}17} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{136} & 17 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}153} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}153 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}108} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{45} & 108 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}17} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{136} & 17 \\ \cline{2-18} 
%  & Glucose & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}153} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}153} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}153 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}153} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}153 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}153} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
%  & Bl\# OOD Pressure & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}5} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{148} & 5 & \multicolumn{1}{r|}{148} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{5} & 148 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}153} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}153 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}5} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{148} & 5 \\ \cline{2-18} 
%  & Skin Thickness & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}50} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{103} & 50 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}153} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}153 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}103} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{50} & 103 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}50} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{103} & 50 \\ \cline{2-18} 
%  & Insulin & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}79} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{74} & 79 & \multicolumn{1}{r|}{74} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{79} & 74 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}153} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}153 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}79} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{74} & 79 \\ \cline{2-18} 
%  & BMI & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{151} & 2 & \multicolumn{1}{r|}{151} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2} & 151 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}153} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}153 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}153} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
%  & Diabetes Pedigree function & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}153} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}153 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}153} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}153 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}43} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{110} & 43 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}153} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
% \multirow{-8}{*}{Pima Diabetes} & Age & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}153} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}153} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}153 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}153} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}153 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}153} & \cellcolor[HTML]{D9EAD3}0 \\ \hline
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}CRIM & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}5} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}95} & \cellcolor[HTML]{F3F3F3}5 & \multicolumn{1}{r|}{95} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}5} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{95} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}5} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}5} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}95} & \cellcolor[HTML]{F3F3F3}5 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}ZN & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}2} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}98} & \cellcolor[HTML]{F3F3F3}2 & \multicolumn{1}{r|}{98} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}2} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{98} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}2} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}2} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}98} & \cellcolor[HTML]{F3F3F3}2 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}INDUS & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}4} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}96} & \cellcolor[HTML]{F3F3F3}4 & \multicolumn{1}{r|}{96} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}4} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{96} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}4} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}4} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}96} & \cellcolor[HTML]{F3F3F3}4 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}CHAS & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}5} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}95} & \cellcolor[HTML]{F3F3F3}5 & \multicolumn{1}{r|}{95} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}5} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{95} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}5} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}5} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}95} & \cellcolor[HTML]{F3F3F3}5 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}NOX & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}RM & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}AGE & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}4} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}96} & \cellcolor[HTML]{F3F3F3}4 & \multicolumn{1}{r|}{96} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}4} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}96} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}4} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}4} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}96} & \cellcolor[HTML]{F3F3F3}4 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}DIS & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}RAD & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}TAX & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}PTRATIO & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}B & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}100} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}100} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
% \multirow{-13}{*}{\cellcolor[HTML]{D9D9D9}Boston Housing} & \cellcolor[HTML]{D9D9D9}LSTAT & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}5} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}95} & \cellcolor[HTML]{F3F3F3}5 & \multicolumn{1}{r|}{95} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}5} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{95} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}5} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}100 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}5} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}95} & \cellcolor[HTML]{F3F3F3}5 \\ \hline
%  & LotArea & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}292} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}292} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}292 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}292} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}292 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}292} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
%  & OverallQual & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}292} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}292} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}292 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}292} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}292 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}292} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
%  & OverallCond & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}292} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}292} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}292 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}292} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}292 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}292} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
%  & TotalBsmtSF & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}5} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{287} & 5 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}287} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{5} & 287 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}292} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}292 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}5} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{287} & 5 \\ \cline{2-18} 
%  & FullBath & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}131} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{161} & 131 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}289} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{3} & 289 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}289} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{3} & 289 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}3} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{289} & 3 \\ \cline{2-18} 
%  & HalfBath & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}185} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{107} & 185 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}107} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{185} & 107 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}107} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{185} & 107 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}185} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{107} & 185 \\ \cline{2-18} 
%  & BedroomAbvGr & \multicolumn{1}{r|}{3} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{289} & 3 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}289} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{3} & 289 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}292} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}292 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}3} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{289} & 3 \\ \cline{2-18} 
%  & TotRmsAbvGrd & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}292} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}292} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}292 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}292} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}292 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}292} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
%  & Fireplaces & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}266} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{26} & 266 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}156} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{136} & 156 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}156} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{136} & 156 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}136} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{156} & 136 \\ \cline{2-18} 
% \multirow{-10}{*}{House Price} & GarageArea & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}17} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{275} & 17 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}275} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{17} & 275 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}292} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}292 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}17} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{275} & 17 \\ \hline
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Pclass & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{CFE2F3}418} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}418} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}418} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D0E0E3}418} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Sex & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}218} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{200} & 218 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Master & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}266} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{152} & 266 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}266} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{152} & 266 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Miss & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}21} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{397} & 21 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}397} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{21} & 397 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Mr & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}340} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{78} & 340 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Mrs & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}178} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{240} & 178 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}240} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{178} & 240 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}240} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{178} & 240 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}178} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{240} & 178 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Others & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}345} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{73} & 345 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}73} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{345} & 73 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}345} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{73} & 345 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Family & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}412} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{6} & 412 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}6} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{412} & 6 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}6} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{412} & 6 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}412} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{6} & 412 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Fare-bin & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}20} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{398} & 20 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}145} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{273} & 145 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}398} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{20} & 398 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}20} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{398} & 20 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Age-bin & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{E6B8AF}0} & \cellcolor[HTML]{E6B8AF}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Ticket\_1 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{E6B8AF}0} & \cellcolor[HTML]{E6B8AF}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Ticket\_2 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}64} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{354} & 64 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Ticket\_3 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}323} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{95} & 323 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}323} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{95} & 323 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Ticket\_4 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}383} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{35} & 383 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Ticket\_C & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}388} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{30} & 388 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{E6B8AF}0} & \cellcolor[HTML]{E6B8AF}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}388} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{30} & 388 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Ticket\_P & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}385} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{33} & 385 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{E6B8AF}0} & \cellcolor[HTML]{E6B8AF}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}33} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{385} & 33 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}385} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{33} & 385 \\ \cline{2-18} 
% \multirow{-17}{*}{\cellcolor[HTML]{D9D9D9}Titanic} & \cellcolor[HTML]{D9D9D9}Ticket\_S & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}418} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}418} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{E6B8AF}0} & \cellcolor[HTML]{E6B8AF}418 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}33} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{385} & 33 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}385} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{33} & 385 \\ \hline
%  & age & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
%  & education & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}95} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2021} & 95 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2021} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{95} & 2021 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}95} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2021} & 95 \\ \cline{2-18} 
%  & balance & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}294} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1822} & 294 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1971} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{145} & 1971 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1822} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{294} & 1822 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}145} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1971} & 145 \\ \cline{2-18} 
%  & day & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
%  & month & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
%  & duration & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
%  & campaign & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
%  & pdays & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1602} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{514} & 1602 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}514} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1602} & 514 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}514} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1602} & 514 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1602} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{514} & 1602 \\ \cline{2-18} 
%  & previous & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1602} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{514} & 1602 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}514} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1602} & 514 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}514} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1602} & 514 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1602} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{514} & 1602 \\ \cline{2-18} 
%  & poutcome & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1603} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{513} & 1603 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2116} & 0 \\ \cline{2-18} 
%  & job\_blue & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1734} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{382} & 1734 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}382} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1734} & 382 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1734} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{382} & 1734 \\ \cline{2-18} 
%  & job\_entrepreneur & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2048} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{68} & 2048 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}68} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2048} & 68 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2048} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{68} & 2048 \\ \cline{2-18} 
%  & job\_housemaid & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2071} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{45} & 2071 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}45} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2071} & 45 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}45} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2071} & 45 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
%  & job\_management & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1641} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{475} & 1641 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}475} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{164} & 475 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
%  & job\_retired & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1971} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{145} & 1971 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}145} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1971} & 145 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
%  & job\_self & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2041} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{75} & 2041 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}75} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2041} & 75 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
%  & job\_services & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1930} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{186} & 1930 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}186} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1930} & 186 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}186} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1930} & 186 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1930} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{186} & 1930 \\ \cline{2-18} 
%  & job\_student & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2046} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{70} & 2046 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}70} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2046} & 70 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}70} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2046} & 70 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
%  & job\_technician & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1781} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{335} & 1781 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}335} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1781} & 335 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}335} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1781} & 335 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1781} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{335} & 1781 \\ \cline{2-18} 
%  & job\_unemployed & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2049} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{67} & 2049 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}67} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2049} & 67 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}67} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2049} & 67 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
%  & job\_unknown & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2102} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{14} & 2102 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}14} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2102} & 14 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}14} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2102} & 14 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2102} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{14} & 2102 \\ \cline{2-18} 
%  & marital\_married & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}916} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1200} & 916 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{916} & 1200 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}916} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1200} & 916 \\ \cline{2-18} 
%  & marital\_single & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1443} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{673} & 1443 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}673} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1443} & 673 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}673} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1443} & 673 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
%  & default\_yes & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2079} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{37} & 2079 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}37} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2079} & 37 & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}2116} & \cellcolor[HTML]{D9EAD3}0 \\ \cline{2-18} 
%  & housing\_yes & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1107} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1009} & 1107 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1009} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1107} & 1009 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1009} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1107} & 1009 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1107} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1009} & 1107 \\ \cline{2-18} 
%  & loan\_yes & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1826} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{290} & 1826 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}2116} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}2116 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}290} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1826} & 290 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1826} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{290} & 1826 \\ \cline{2-18} 
%  & contact\_telephone & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1946} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{170} & 1946 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}170} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1946} & 170 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}170} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1946} & 170 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1946} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{170} & 1946 \\ \cline{2-18} 
% \multirow{-28}{*}{Bank Customer} & contact\_unknown & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1650} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{466} & 1650 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}466} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1650} & 466 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}466} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{1650} & 466 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}1650} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{466} & 1650 \\ \hline
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Age & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}187} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{13} & 187 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}200 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}192} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{8} & 192 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}194} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{6} & 194 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Job & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}44} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{156} & 44 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}156} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{44} & 156 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}195} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{5} & 195 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}171} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{29} & 171 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Credit amount & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}154} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{46} & 154 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}39} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{161} & 39 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}166} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{34} & 166 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}196} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{4} & 196 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Duration & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}183} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{17} & 183 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}48} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{152} & 48 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}142} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{58} & 142 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}198} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{2} & 198 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Sex\_female & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}145} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{55} & 145 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}55} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{145} & 55 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}200 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & 200 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Sex\_male & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}55} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{145} & 55 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}145} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{55} & 145 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}200 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & 200 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Housing\_free & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}182} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{18} & 182 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}18} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{182} & 18 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}18} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}182} & \cellcolor[HTML]{F3F3F3}18 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}182} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{18} & 182 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Housing\_own & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}57} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{143} & 57 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}143} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{57} & 143 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}200 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & 200 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Housing\_rent & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}161} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{39} & 161 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}39} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{161} & 39 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}39} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{161} & 39 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}161} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{39} & 161 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Saving accounts\_little & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}73} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{127} & 73 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}127} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{73} & 127 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}127} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{73} & 127 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & 200 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Saving accounts\_moderate & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}186} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{14} & 186 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}14} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{186} & 14 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}14} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{186} & 14 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}186} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{14} & 186 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Saving accounts\_quite rich & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}188} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{12} & 188 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}200 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}12} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{188} & 12 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}188} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{12} & 188 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Saving accounts\_rich & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}194} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{6} & 194 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}6} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{194} & 6 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}200 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}194} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{6} & 194 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Checking account\_little & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}135} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{65} & 135 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}65} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{135} & 65 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}65} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{135} & 65 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & 200 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Checking account\_moderate & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}157} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{43} & 157 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}43} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{157} & 43 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}43} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{157} & 43 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}157} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{43} & 157 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Checking account\_rich & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}192} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{8} & 192 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}8} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{192} & 8 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}8} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{192} & 8 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}192} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{8} & 192 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Purpose\_business & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}180} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{20} & 180 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}20} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{180} & 20 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}20} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{180} & 20 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & 200 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Purpose\_car & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}128} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{72} & 128 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}72} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{128} & 72 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}72} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{128} & 72 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & 200 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Purpose\_domestic appliances & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}197} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{3} & 197 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}3} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{197} & 3 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}3} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{197} & 3 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & 200 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Purpose\_education & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}194} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{6} & 194 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}6} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{194} & 6 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}6} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{194} & 6 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & 200 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Purpose\_furniture/equipment & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}163} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{37} & 163 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}37} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{163} & 37 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}200 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{0} & 200 \\ \cline{2-18} 
% \cellcolor[HTML]{D9D9D9} & \cellcolor[HTML]{D9D9D9}Purpose\_radio/TV & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}143} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{57} & 143 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}57} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{143} & 57 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}57} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{143} & 57 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}143} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{57} & 143 \\ \cline{2-18} 
% \multirow{-23}{*}{\cellcolor[HTML]{D9D9D9}German Credit} & \cellcolor[HTML]{D9D9D9}Purpose\_repairs & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}197} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{3} & 197 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}3} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{197} & 3 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}200} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{\cellcolor[HTML]{F4CCCC}0} & \cellcolor[HTML]{F4CCCC}200 & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D2E9}197} & \multicolumn{1}{r|}{0} & \multicolumn{1}{r|}{3} & 197 \\ \hline
% % \end{tabular}
%   \footnotesize
     
%   { * Here, \violet{cells} represent total out-of-distribution (\# OOD) values detected for a feature, \cyan{cells} represent total missing (\# Miss) values for that particular feature,  \red{cells} denote where data precondition is violated for all test data examples  and \green{cells} indicate where data precondition is satisfied for all test data examples.}
%   \label{tab:rq2table}
% \end{table*}

==> tables/rq3table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[htbp]
\tiny
\centering
\caption{Localize problem in model architecture from data precondition violation}
\begin{tabular}{|llrrrrrl|}
\hline
\rowcolor[HTML]{D9D9D9} 
Datasets & Models & \multicolumn{1}{l}{\cellcolor[HTML]{D9D9D9}Loss} & \multicolumn{1}{l}{\cellcolor[HTML]{D9D9D9}Accuracy/ MAE} & \# Features & \# Violation & \multicolumn{1}{l}{\cellcolor[HTML]{D9D9D9}\# Violation/ total (\%)} & Problem in model architecture \\ \hline
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{Model\#1} & \multicolumn{1}{r|}{0.49} & \multicolumn{1}{r|}{77.08\%} & \multicolumn{1}{r|}{} & \multicolumn{1}{r|}{306} & \multicolumn{1}{r|}{25.00\%} & \multicolumn{1}{l|}{no issue detected} \\ \cline{2-4} \cline{6-8} 
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{Model\#2} & \multicolumn{1}{r|}{5.38} & \multicolumn{1}{r|}{65.10\%} & \multicolumn{1}{r|}{} & \multicolumn{1}{r|}{86} & \multicolumn{1}{r|}{93.00\%} & \multicolumn{1}{l|}{layer 3: activation:`tanh'} \\ \cline{2-4} \cline{6-8} 
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{Model\#3} & \multicolumn{1}{r|}{5.31} & \multicolumn{1}{r|}{65.49\%} & \multicolumn{1}{r|}{} & \multicolumn{1}{r|}{1019} & \multicolumn{1}{r|}{83.00\%} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}layer 3: activation:`relu'} \\ \cline{2-4} \cline{6-8} 
\multicolumn{1}{|l|}{\multirow{-4}{*}{Pima Diabetes}} & \multicolumn{1}{l|}{Model\#4} & \multicolumn{1}{r|}{0.48} & \multicolumn{1}{r|}{77.47\%} & \multicolumn{1}{r|}{\multirow{-4}{*}{10}} & \multicolumn{1}{r|}{151} & \multicolumn{1}{r|}{12.00\%} & \multicolumn{1}{l|}{no issue detected} \\ \hline
\rowcolor[HTML]{F3F3F3} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{F3F3F3}} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}Model\#1} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}28.73} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}3.96} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}25} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}2.00\%} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}no issue detected} \\ \cline{2-4} \cline{6-8} 
\rowcolor[HTML]{F3F3F3} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{F3F3F3}} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}Model\#2} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}532.36} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}21.12} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}1300} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}100.00\%} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}layer 3: activation:`tanh'} \\ \cline{2-4} \cline{6-8} 
\rowcolor[HTML]{F3F3F3} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{F3F3F3}} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}Model\#3} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}40.67} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}4.78} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}1300} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}100.00\%} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}layer 3: activation:`relu'} \\ \cline{2-4} \cline{6-8} 
\rowcolor[HTML]{F3F3F3} 
\multicolumn{1}{|l|}{\multirow{-4}{*}{\cellcolor[HTML]{F3F3F3}Boston Housing}} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}Model\#4} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}32.59} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}3.69} & \multicolumn{1}{r|}{\multirow{-4}{*}{\cellcolor[HTML]{F3F3F3}13}} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}25} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}2.00\%} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}no issue detected} \\ \hline
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{Model\#1} & \multicolumn{1}{r|}{0.33} & \multicolumn{1}{r|}{85.22\%} & \multicolumn{1}{r|}{} & \multicolumn{1}{r|}{607} & \multicolumn{1}{r|}{21.00\%} & \multicolumn{1}{l|}{no issue detected} \\ \cline{2-4} \cline{6-8} 
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{Model\#2} & \multicolumn{1}{r|}{0.22} & \multicolumn{1}{r|}{89.77\%} & \multicolumn{1}{r|}{} & \multicolumn{1}{r|}{2571} & \multicolumn{1}{r|}{88.00\%} & \multicolumn{1}{l|}{layer 3: activation:`tanh'} \\ \cline{2-4} \cline{6-8} 
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{Model\#3} & \multicolumn{1}{r|}{8.41} & \multicolumn{1}{r|}{45.45\%} & \multicolumn{1}{r|}{} & \multicolumn{1}{r|}{2596} & \multicolumn{1}{r|}{88.00\%} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}layer 3: activation:`relu'} \\ \cline{2-4} \cline{6-8} 
\multicolumn{1}{|l|}{\multirow{-4}{*}{House Price}} & \multicolumn{1}{l|}{Model\#4} & \multicolumn{1}{r|}{0.25} & \multicolumn{1}{r|}{87.50\%} & \multicolumn{1}{r|}{\multirow{-4}{*}{10}} & \multicolumn{1}{r|}{349} & \multicolumn{1}{r|}{12.00\%} & \multicolumn{1}{l|}{no issue detected} \\ \hline
\rowcolor[HTML]{F3F3F3} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{F3F3F3}} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}Model\#1} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}0.07} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}96.77\%} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}2838} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}39.00\%} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}no issue detected} \\ \cline{2-4} \cline{6-8} 
\rowcolor[HTML]{F3F3F3} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{F3F3F3}} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}Model\#2} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}5.92} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}61.61\%} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}4719} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}66.00\%} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}layer 3: activation:`tanh'} \\ \cline{2-4} \cline{6-8} 
\rowcolor[HTML]{F3F3F3} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{F3F3F3}} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}Model\#3} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}0.05} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}97.66\%} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}4792} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}67.00\%} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}layer 3: activation:`relu'} \\ \cline{2-4} \cline{6-8} 
\rowcolor[HTML]{F3F3F3} 
\multicolumn{1}{|l|}{\multirow{-4}{*}{\cellcolor[HTML]{F3F3F3}Titanic}} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}Model\#4} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}0.20} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}97.02\%} & \multicolumn{1}{r|}{\multirow{-4}{*}{\cellcolor[HTML]{F3F3F3}17}} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}1112} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}16.00\%} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}no issue detected} \\ \hline
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{Model\#1} & \multicolumn{1}{r|}{0.41} & \multicolumn{1}{r|}{81.30\%} & \multicolumn{1}{r|}{} & \multicolumn{1}{r|}{37577} & \multicolumn{1}{r|}{63.00\%} & \multicolumn{1}{l|}{no issue detected} \\ \cline{2-4} \cline{6-8} 
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{Model\#2} & \multicolumn{1}{r|}{0.42} & \multicolumn{1}{r|}{81.90\%} & \multicolumn{1}{r|}{} & \multicolumn{1}{r|}{31010} & \multicolumn{1}{r|}{52.00\%} & \multicolumn{1}{l|}{layer 3: activation:`tanh'} \\ \cline{2-4} \cline{6-8} 
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{Model\#3} & \multicolumn{1}{r|}{4.56} & \multicolumn{1}{r|}{69.60\%} & \multicolumn{1}{r|}{} & \multicolumn{1}{r|}{30038} & \multicolumn{1}{r|}{52.00\%} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}layer 3: activation:`relu'} \\ \cline{2-4} \cline{6-8} 
\multicolumn{1}{|l|}{\multirow{-4}{*}{Bank Customer}} & \multicolumn{1}{l|}{Model\#4} & \multicolumn{1}{r|}{0.41} & \multicolumn{1}{r|}{80.70\%} & \multicolumn{1}{r|}{\multirow{-4}{*}{23}} & \multicolumn{1}{r|}{20484} & \multicolumn{1}{r|}{35.00\%} & \multicolumn{1}{l|}{layer 4: activation: `sigmoid'} \\ \hline
\rowcolor[HTML]{F3F3F3} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{F3F3F3}} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}Model\#1} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}0.05} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}99.00\%} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}3495} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}76.00\%} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}no issue detected} \\ \cline{2-4} \cline{6-8} 
\rowcolor[HTML]{F3F3F3} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{F3F3F3}} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}Model\#2} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}0.15} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}99.00\%} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}1504} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}33.00\%} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}layer 3: activation:`tanh'} \\ \cline{2-4} \cline{6-8} 
\rowcolor[HTML]{F3F3F3} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{F3F3F3}} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}Model\#3} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}0.15} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}99.00\%} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}2379} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}52.00\%} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}layer 3: activation:`relu'} \\ \cline{2-4} \cline{6-8} 
\rowcolor[HTML]{F3F3F3} 
\multicolumn{1}{|l|}{\multirow{-4}{*}{\cellcolor[HTML]{F3F3F3}German Credit}} & \multicolumn{1}{l|}{\cellcolor[HTML]{F3F3F3}Model\#4} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}0.06} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}99.00\%} & \multicolumn{1}{r|}{\multirow{-4}{*}{\cellcolor[HTML]{F3F3F3}28}} &  \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}4359} & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}95.00\%} & no issue detected \\ \hline
\end{tabular}
\label{tab:rq3table}
\end{table*}










==> tables/rq4table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]


\begin{table*}[htbp]
  \setlength{\parskip}{.1cm}
%	\setlength{\intextsep}{.1cm plus .1cm minus 1.cm} 
\setlength{\belowcaptionskip}{.05cm}
\tiny
\centering
\caption{Data precondition violation to justify prediction with test data}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|r|r|r|r|r|rrr|rrrr|}
\hline
\rowcolor[HTML]{D9D9D9} 
\cellcolor[HTML]{D9D9D9}                               & \cellcolor[HTML]{D9D9D9}                         & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}}                       & \cellcolor[HTML]{D9D9D9}                           & \cellcolor[HTML]{D9D9D9}                              & \cellcolor[HTML]{D9D9D9}                               & \multicolumn{1}{l|}{\cellcolor[HTML]{D9D9D9}}                               & \multicolumn{3}{c|}{\cellcolor[HTML]{D9D9D9}Ground Truth}                                                                                    & \multicolumn{4}{c|}{\cellcolor[HTML]{D9D9D9}Data Precondition Warning}                                                                                                                            \\ \cline{8-14} 
\rowcolor[HTML]{D9D9D9} 
\multirow{-2}{*}{\cellcolor[HTML]{D9D9D9}Dataset}      & \multirow{-2}{*}{\cellcolor[HTML]{D9D9D9}Models} & \multicolumn{1}{l|}{\multirow{-2}{*}{\cellcolor[HTML]{D9D9D9}Loss}} & \multirow{-2}{*}{\cellcolor[HTML]{D9D9D9}Accuracy} & \multirow{-2}{*}{\cellcolor[HTML]{D9D9D9}\# Features} & \multirow{-2}{*}{\cellcolor[HTML]{D9D9D9}\# Violation} & \multicolumn{1}{l|}{\multirow{-2}{*}{\cellcolor[HTML]{D9D9D9}\# Satisfied}} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}\# Correct} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}\# Wrong} & FP                         & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}\# Correct} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}\# Wrong} & \multicolumn{1}{r|}{\cellcolor[HTML]{D9D9D9}FP}  & FP rate                      \\ \hline
                                                       & Model\#1                                         & 0.49                                                                & 77.08\%                                            &                                                       & 315                                                    & 909                                                                         & \multicolumn{1}{r|}{119}                                & \multicolumn{1}{r|}{34}                               & 34                         & \multicolumn{1}{r|}{147}                                & \multicolumn{1}{r|}{6}                                & \multicolumn{1}{r|}{34}                          & 0.22                         \\ \cline{2-4} \cline{6-14} 
                                                       & Model\#2                                         & 5.38                                                                & 65.10\%                                            &                                                       & 1185                                                   & 39                                                                          & \multicolumn{1}{r|}{99}                                 & \multicolumn{1}{r|}{54}                               & 54                         & \multicolumn{1}{r|}{37}                                 & \multicolumn{1}{r|}{116}                              & \multicolumn{1}{r|}{78}                          & 0.51                         \\ \cline{2-4} \cline{6-14} 
                                                       & Model\#3                                         & 5.31                                                                & 65.49\%                                            &                                                       & 1021                                                   & 203                                                                         & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}98}         & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}55}       & \cellcolor[HTML]{FFFFFF}55 & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}22}         & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}131}      & \multicolumn{1}{r|}{90}                          & 0.59                         \\ \cline{2-4} \cline{6-14}                                                       
\parbox[t]{2mm}{\multirow{-4}{*}{\rotatebox[origin=c]{45}{Pima}}}                        & Model\#4                                         & 0.48                                                                & 77.47\%                                            & \multirow{-4}{*}{10}                                  & 334                                                    & 890                                                                         & \multicolumn{1}{r|}{111}                                & \multicolumn{1}{r|}{42}                               & 42                         & \multicolumn{1}{r|}{147}                                & \multicolumn{1}{r|}{6}                                & \multicolumn{1}{r|}{44}                          & 0.29                         \\ \hline
\rowcolor[HTML]{F3F3F3} 
\cellcolor[HTML]{F3F3F3}                               & Model\#1                                         & 0.33                                                                & 85.22\%                                            & \cellcolor[HTML]{F3F3F3}                              & 349                                                    & 2,571                                                                       & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}147}        & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}145}      & 145                        & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}269}        & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}23}       & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}126} & 0.43                         \\ \cline{2-4} \cline{6-14} 
\rowcolor[HTML]{F3F3F3} 
\cellcolor[HTML]{F3F3F3}                               & Model\#2                                         & 0.22                                                                & 89.77\%                                            & \cellcolor[HTML]{F3F3F3}                              & 2571                                                   & 349                                                                         & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}147}        & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}145}      & 145                        & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}98}         & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}194}      & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}205} & 0.70                         \\ \cline{2-4} \cline{6-14} 
\rowcolor[HTML]{F3F3F3} 
\cellcolor[HTML]{F3F3F3}                               & Model\#3                                         & 8.41                                                                & 45.45\%                                            & \cellcolor[HTML]{F3F3F3}                              & 2596                                                   & 324                                                                         & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}145}        & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}147}      & 147                        & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}98}         & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}194}      & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}87}  & 0.30                         \\ \cline{2-4} \cline{6-14} 
\rowcolor[HTML]{F3F3F3}
\parbox[t]{2mm}{\multirow{-4}{*}{\rotatebox[origin=c]{45}{\cellcolor[HTML]{F3F3F3}HousePrice}}}  & Model\#4                                         & 0.25                                                                & 87.50\%                                            & \multirow{-4}{*}{\cellcolor[HTML]{F3F3F3}10}          & 349                                                    & 2,571                                                                       & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}147}        & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}145}      & 145                        & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}269}        & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}23}       & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}126} & 0.43                         \\ \hline
                                                       & Model\#1                                         & 0.41                                                                & 81.30\%                                            &                                                       & 34004                                                  & 25,244                                                                      & \multicolumn{1}{r|}{1060}                               & \multicolumn{1}{r|}{1056}                             & 1056                       & \multicolumn{1}{r|}{455}                                & \multicolumn{1}{r|}{1661}                             & \multicolumn{1}{r|}{993}                         & \cellcolor[HTML]{FFFFFF}0.47 \\ \cline{2-4} \cline{6-14} 
                                                       & Model\#2                                         & 0.42                                                                & 81.90\%                                            &                                                       & 31,010                                                 & 28238                                                                       & \multicolumn{1}{r|}{1060}                               & \multicolumn{1}{r|}{1056}                             & 1056                       & \multicolumn{1}{r|}{167}                                & \multicolumn{1}{r|}{1949}                             & \multicolumn{1}{r|}{1,049}                       & \cellcolor[HTML]{FFFFFF}0.50 \\ \cline{2-4} \cline{6-14} 
                                                       & Model\#3                                         & 4.56                                                                & 69.60\%                                            &                                                       & 30038                                                  & 29,210                                                                      & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1060}       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1056}     & 1056                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}122}        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1994}     & \multicolumn{1}{r|}{1,066}                       & \cellcolor[HTML]{FFFFFF}0.50 \\ \cline{2-4} \cline{6-14} 
\parbox[t]{2mm}{\multirow{-4}{*}{\rotatebox[origin=c]{45}{BankCust.}}}                        & Model\#4                                         & 0.41                                                                & 80.70\%                                            & \multirow{-4}{*}{22}                                  & 20484                                                  & 38,764                                                                      & \multicolumn{1}{r|}{1060}                               & \multicolumn{1}{r|}{1056}                             & 1056                       & \multicolumn{1}{r|}{1879}                               & \multicolumn{1}{r|}{237}                              & \multicolumn{1}{r|}{1,073}                       & \cellcolor[HTML]{FFFFFF}0.51 \\ \hline
\rowcolor[HTML]{F3F3F3} 
\cellcolor[HTML]{F3F3F3}                               & Model\#1                                         & 0.05                                                                & 99.00\%                                            & \cellcolor[HTML]{F3F3F3}                              & 1205                                                   & 3,195                                                                       & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}198}        & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}2}        & 2                          & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}53}         & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}147}      & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}145} & 0.73                         \\ \cline{2-4} \cline{6-14} 
\rowcolor[HTML]{F3F3F3} 
\cellcolor[HTML]{F3F3F3}                               & Model\#2                                         & 0.15                                                                & 99.00\%                                            & \cellcolor[HTML]{F3F3F3}                              & 1277                                                   & 3,123                                                                       & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}198}        & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}2}        & 2                          & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}28}         & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}172}      & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}170} & 0.85                         \\ \cline{2-4} \cline{6-14} 
\rowcolor[HTML]{F3F3F3} 
\cellcolor[HTML]{F3F3F3}                               & Model\#3                                         & 0.15                                                                & 99.00\%                                            & \cellcolor[HTML]{F3F3F3}                              & 899                                                    & 3,501                                                                       & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}198}        & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}2}        & 2                          & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}65}         & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}135}      & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}133} & 0.67                         \\ \cline{2-4} \cline{6-14} 
\rowcolor[HTML]{F3F3F3} 
\parbox[t]{2mm}{\multirow{-4}{*}{\rotatebox[origin=c]{45}{\cellcolor[HTML]{F3F3F3}GermanCr.}}} & Model\#4                                         & 0.06                                                                & 99.00\%                                            & \multirow{-4}{*}{\cellcolor[HTML]{F3F3F3}28}          & 891                                                    & 3,509                                                                       & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}198}        & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}2}        & 2                          & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}66}         & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}134}      & \multicolumn{1}{r|}{\cellcolor[HTML]{F3F3F3}132} & 0.66                         \\ \hline
\end{tabular}}
\label{tab:rq4table}
\end{table*}
